PITA: Preference-Guided Inference-Time Alignment for LLM Post-Training

Inference-time alignment enables large language models (LLMs) to generate outputs aligned with end-user preferences without further training. Recent post-training methods achieve this by using small guidance models to modify token generation during inference. These methods typically optimize a reward function KL-regularized by the original LLM taken as the reference policy. A critical limitation, however, is their dependence on a pre-trained reward model, which requires fitting to human preference feedback--a potentially unstable process. In contrast, we introduce PITA, a novel framework that integrates preference feedback directly into the LLM's token generation, eliminating the need for a reward model. PITA learns a small preference-based guidance policy to modify token probabilities at inference time without LLM fine-tuning, reducing computational cost and bypassing the pre-trained reward model dependency. The problem is framed as identifying an underlying preference distribution, solved through stochastic search and iterative refinement of the preference-based guidance model. We evaluate PITA across diverse tasks, including mathematical reasoning and sentiment classification, demonstrating its effectiveness in aligning LLM outputs with user preferences.

==> arxiv/sections/OLD-experiments.tex <==
\section{Experiments}\label{sec:experiments}
We adopt the experimental approach by Q\#. Since Q\# is one of the approaches we compare the performance of PITA against, we use the same base models, and datasets. In this section, we provide a brief overview of the experimental setup. Additional details on datasets, training, and evaluation criterion are provided in Appendix~\ref{app:experiments}.
All our experiments were run on machines with one NVIDIA A100 80 GB GPU. Our code is available at \url{https://anonymous.4open.science/r/pref-sharp-D223}



%\paragraph{OBJECTIVE:} 
We empirically evaluate the proposed \textbf{PITA} algorithm on mathematics reasoning tasks and compare it against a strong reward-model baseline. Our study focuses on three key questions: 1) Does PITA improve task accuracy (\textit{pass@1} and \textit{maj@8}) over a baseline that performs post-training Q\# with a learnt preference reward model? 2) Does the KL divergence to the reference policy %(\(\pi_{\text{ref}}\))
remain controlled? 3) How well does the learned reward model discriminate between correct and incorrect generations?

\subsection{Experimental Setup}\label{subsec:setup}


% \textbf{Dataset.} All experiments use the \textsc{GSM8K} benchmark\,\citep{cobbe2021gsm8k}—a collection of $8\,500$ grade-school mathematics problems with short free-form answers—split into 7.5k train and 1k test samples.
\textbf{Datasets.} We evaluate our algorithm on arithmetic reasoning dataset GSM8k~\cite{cobbe2021training}.
GSM8K (Grade School Math 8K) is a dataset containing 8.5K high-quality, linguistically diverse math word problems aimed at grade school level. Designed for question answering tasks, these problems require 2 to 8 steps and involve basic arithmetic operations. For test set evaluation, the entire GSM8K test set and a subset of the MATH-500 datasets chosen at random are used to check the performance of the trained PITA model~\cite{lightman2023let,wang2023math}.

\textbf{Models.} We use the Llama 3~\cite{grattafiori2024llama} family of models to train our preference function since they are fairly competitive in arithmetic reasoning tasks~\cite{zhou2025q}.

\textbf{Metrics.} We report \emph{pass@1} (exact-match accuracy of the highest-ranking sample), \emph{maj1@8} (majority-vote accuracy over 8 samples), and the forward KL divergence $\text{KL}(\pi\,\Vert\,\pi_{\text{ref}})$ computed on the \textsc{GSM8K} test set. Lower KL indicates closer adherence to the reference policy.



\textbf{Algorithms:} We make a comparison of the performance of the following algorithms on the GSM8K dataset to the base reference model $\pi_{\mathrm{ref}}$. \\
%\vspace{0.01in}
\textbf{Q\#:} The trained Q\# model is evaluated for it's accuracy on the GSM8K dataset.\\
%\vspace{0.01in}
%\vspace{-0.01in}\\
\textbf{Q\#-HF.} We first train a reward model using preference data derived from the GSM8K dataset. This reward model is then used in the Q\# algorithm to train a final model. \\
%\vspace{-0.01in}\\
\textbf{PITA (ours).} The iterative approach described in Section~\ref{sec:PITA} is used to learn an optimal soft-Q function from preference data derived from the GSM8K dataset. The final model, induced by the learned $Q$-function, is then evaluated.\\
%\vspace{-0.01in}\\
\textbf{Training details.} Each optimisation run uses a single NVIDIA~A100 card. PITA trains for $10$ policy-evaluation/optimisation cycles of $1$-epoch each with learning rate $2\times10^{-5}$ and context length~$4096$. The baseline uses identical hyper-parameters.\\



\textbf{Main Results:}
In Table~\ref{tab:gsm8k_main}, we compare the performance of the above algorithms. The reference model $\pi_{\mathrm{ref}}$ is chosen to be the Llama 3 8B model. We observe that PITA performs significantly better than Llama3 on both \textbf{pass@1} accuracy as well as \textbf{maj@8} evaluation metrics. In addition, the gap between PITA and $Q\#$ seems to be considerably close. 
%We believe that the difference in performance is an artifact of $Q\#$ 
% \begin{table}[h]
%     \centering
%     \label{tab:gsm8k_main}
%     \begingroup
%     \setlength{\tabcolsep}{6pt}
%     \begin{tabular}{lccc}
%         \toprule
%         Method & pass@1$\uparrow$ & maj@8$\uparrow$ & KL$\downarrow$ \\
%         \midrule
%         \pi_{\mathrm{ref}} & \placeholder{} & \placeholder{} & \placeholder{} \\
%         Q\# & \placeholder{} & \placeholder{} & \placeholder{} \\
%         Q\#-HF & \placeholder{} & \placeholder{} & \placeholder{} \\
%         PITA (ours) & \placeholder{} & \placeholder{} & \placeholder{} \\
%         \bottomrule
%     \end{tabular}
%     \endgroup
%     \caption{Performance on the \textsc{GSM8K} \emph{test} split. Placeholder numbers \placeholder{} will be replaced once experiments finish.}
% \end{table}

\begin{table}[h]
    \centering
    \caption{Performance on the \textsc{GSM8K} \emph{test} split.}
    \label{tab:gsm8k_main}
    \begingroup
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Algorithm} & \textbf{pass@1} $\uparrow$ & \textbf{maj@8} $\uparrow$ & \textbf{KL}  \\
        %Algorithm & pass@1$\uparrow$ & maj@8$\uparrow$ & KL$\downarrow$ \\
        \midrule
        $\pi_{\mathrm{ref}}$ & 69 & 85 & - \\
        Q\# & 78.4 & 88.1 & 2.65 \\
        Q\#-HF & --- & --- & --- \\
        PITA (ours)  & 74.8 & 86.1 & --- \\
        \bottomrule
    \end{tabular}
    \endgroup
\end{table}




\textbf{Reward-Model Calibration:}
Figure~\ref{fig:reward_hist} contrasts reward scores assigned by the BT model to
correct versus incorrect generations produced by the baseline. A larger separation
indicates stronger alignment between reward and task success.

\begin{figure}[h]
    \centering
    % Replace the file name with the actual histogram once available.
    \includegraphics[width=0.4\linewidth]{neurips2025/figures/histograms/reward_histogram_OOD_sigmoid.pdf}
    \caption{Distribution of BT reward scores for correct (green) and incorrect (red) \textsc{GSM8K} answers under the MLE\,+\,Q\# baseline.}
    \label{fig:reward_hist}
\end{figure}

\textbf{Discussion:}
We anticipate that PITA will outperform the MLE\,+\,Q\# baseline on both accuracy metrics while maintaining a comparable or lower KL divergence, demonstrating that iterative policy optimisation with sparse rewards is more sample-efficient than single-stage MLE fine-tuning. Additional tasks appear in Appendix~\ref{app:experiments}.




%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%




==> arxiv/sections/OLD-preliminaries.tex <==
\vspace{-0.2cm}
\section{Preliminaries}
We begin by introducing the finite-horizon Markov Decision Process (MDP) framework that formalizes the generation process of language modeling.

A finite-horizon MDP is formulated as $\mathcal{M} = (\mathcal{P}, \mathcal{S}, \mathcal{A}, T, \rho)$, $\mathcal{S}$ is a finite set of states, $\mathcal{A}$ is a set of actions, $\mathcal{P}: \mathcal{S} \times \mathcal{A} \rightarrow \Delta(\mathcal{S})$ is the transition kernel, $T \in \mathbb{N}$ is the maximal length of the episode, $\rho$ denotes the starting state distribution. A policy in MDPs, denoted by $\pi : \mathcal{S} \rightarrow \Delta(\mathcal{A})$, maps each state to a distribution over actions. The dynamics of the MDP can be described as follows. Initially, the starting state $s_0$ is sampled from the initial distribution $\rho$. At each step $t$, the policy selects an action $a_t$ based on the current state $s_t$. The process transitions to the next state $s_{t+1}$, which is sampled from the distribution $\mathcal{P}(\cdot \mid s_t, a_t)$. This process continues until a termination condition is met within the horizon length $T$.

% \textcolor{orange}{::Do we want to start the paragraph saying this is our motivation? Some sort of connecting text to the paragraph above.::}
\textbf{LLMs as Deterministic MDPs:} In text generation applications using an LLM, $\pi$ is the LLM's policy to choose the next token (action) given the current sequence of tokens (state). The transition kernel is deterministic; as each new state state is obtained by concatenating the previous tokens with the current token chosen by the policy. Each sentence generated by the policy is termed a trajectory $\tau = (s_0,a_0,s_1,a_1,\cdots)$, where $s_0 := x$ is the initial instruction sampled from the starting state distribution $\rho$, and $a_t \sim \pi(\cdot |s_t)$. Therefore, at each step $t$, the state $s_t = (x | a_{1:t-1})$ consists of the instruction $x$ and tokens generated upto $t-1$. The generation process ends when the LLM policy samples a special end-of-sequence token or the trajectory reaches a predefined length limit, characterized by $T$. The score of a trajectory generated by the LLM is defined using a reward function
% \textcolor{orange}{$\mathrm{s}(\tau) = r(s_{T-1},a_{T-1})$ :: this notation is a little confusing because you skipped directly to writing it in terms of the reward at the terminal node::} 
$r(s,a):\mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$. The reward function is typically sparse with $r(s_t,a_t) = 0 \forall t \in [T-2]$ quantifiying the desirability of the final output of the LLM for the given instruction $x$. An LLM policy can be learned using T-horizon reinforcement learning by maximizing the expected reward for a given policy defined as $J(\pi) = \mathbb{E}_{\tau \sim \pi} [R(\tau)] = \mathbb{E}_{x \sim \rho}[V^{\pi}(x)]$, where $V^{\pi}(s) = \mathbb{E}_{\pi} \left[ \sum_{t}^T r(s_t,a_t) | s_t = s \right]$ is the value of a state $s$ under policy $\pi$. Similarly, the state-action value function and the advantage function for a state-action pair $(s,a)$ are given by 
$Q^{\pi}(s,a) = \mathbb{E}_{\pi} \left[ \sum_{t}^T r(s_t,a_t) | s_t = s, a_t = a  \right]$, and $A^{\pi(s,a)} = Q^{\pi(s,a)} - V^{\pi(s)}$ respectively.

RLHF and DPO are few standard approaches to align LLMs with human preference data. The RLHF pipeline consists of three steps: a supervised fine-tuning phase where a pre-trained LLM is fine-tuned with supervised learning for downstream task(s) to obtain a model $\pi_{ref}$, a reward modeling phase to estimate a reward function for the LLMs generations, and a fine-tuning phase to find the optimal policy which maximizes the expected reward while not deviating too far from the reference model $\pi_{\mathrm{ref}}$.

\textbf{Reward Modeling:} The reference model $\pi_{\mathrm{ref}}$ is prompted with an instruction $x$ to obtain an answer pair $(y_1,y_2)$. The completions are presented to human annotators who express their preference for one answer over the other, denotes as $y_w \succ y_l | x$ where $y_w$ and $y_l$ denote the preferred and dispreferred completions respectively. The preferences are assumed to be generated according to the Bradley-Terry model~\cite{bradley1952rank}, given by
\begin{equation}
    \mathcal{P}^*(y_w \succ y_l) = \sigma(r^*(x,y_w) - r^*(x,y_l)).
\end{equation}
where $r^*(\cdot,\cdot)$ is latent reward model unknown to the LLM. Assuming acccess to an offline dataset $\mathcal{D} = {(x^{(i)},y_w^{(i)},y_l^{(i)})}_{i=1}^n$ of preference information generated from $\mathcal{P}^*$, the reward model is parameterized as $r_{\theta}(x,y)$ and estimated via maximum likelihood. The estimation problem is formalized as a binary classification problem with the negative log-likelihood loss given by
\begin{equation}
    \mathcal{L}(r_{\theta},\mathcal{D}) = - \mathbb{E}_{(x,y_w,y_l)} \left[ \log{\sigma(r_{\theta}(x,y_w) - r_{\theta}(x,y_l))}\right]
\end{equation}

\textbf{RL Fine-Tuning:} The reference model $\pi_{\mathrm{ref}}$ is fine-tuned with the learned reward function $r_{\theta}$ which is posed as the following KL-regularized constraint optimization problem

\begin{equation}
   \max_{\pi} \mathbb{E}_{x \sim \mathcal{D},\, y \sim \pi(y \mid x)} \left[ r_\theta(x, y) \right] - \eta \mathrm{KL} \left[ \pi(y \mid x) \,\|\, \pi_{\mathrm{ref}}(y \mid x) \right] 
\end{equation}

where $\eta$ is a parameter that controls the deviation of the learned $\pi$ from the reference policy $\pi_{\mathrm{ref}}$, and the KL divergence is defined as $\mathrm{KL}(p || q) = \mathbb{E}_{z \sim p} \left[ \log{p(z)/q(z)}\right]$.

\textbf{DPO:} In ~\cite{rafailov2023direct},the RL fine-tuning step is solved as supervised learning problem to directly learn the optimal policy using preference information. The key idea is that, the optimal policy as obtained by solving the KL-constrained reward maximization objective is a function of the implicit reward model, and has the following form:
\begin{equation}
    \pi^*_r(y \mid x) = \frac{1}{Z(x)} \pi_{\mathrm{ref}}(y \mid x) \exp\left( \frac{1}{\eta} r^*(x, y) \right) 
\end{equation}

where $Z(x) = \sum_y \pi_{\mathrm{ref}}(y|x) \exp(\frac{1}{\eta}r^*(x,y))$ is the partition function. Although, estimation of the parition function is difficult, DPO circumvents this challenge by expression the BT preference model as a function of the optimal policy $\pi^*$ given by
\begin{equation}
    \mathcal{P}^*(y_1 \succ y_2 \mid x) = \frac{1}{1 + \exp\left( \eta \log \frac{\pi^*(y_2 \mid x)}{\pi_{\mathrm{ref}}(y_2 \mid x)} - \eta \log \frac{\pi^*(y_1 \mid x)}{\pi_{\mathrm{ref}}(y_1 \mid x)} \right)}
\end{equation}

Similar to the reward modeling approach, under the above reformulation of the preference model, the policy objective is defined as:
\begin{equation}
\mathcal{L}_{\text{DPO}}(\pi; \pi_{\text{ref}}) = - \mathbb{E}_{(x, y_w, y_l) \sim \mathcal{D}} \left[ 
\log \sigma \left( 
\beta \log \frac{\pi(y_w \mid x)}{\pi_{\text{ref}}(y_w \mid x)} - 
\beta \log \frac{\pi(y_l \mid x)}{\pi_{\text{ref}}(y_l \mid x)} 
\right) 
\right].
\end{equation}


==> arxiv/sections/OLD-test-time-with-preference.tex <==


\section{PITA: Preference-Guided Inference-Time Alignment} \label{sec:ra-rlhf}


In this section, we present our algorithm for the test time scaling of LLMs using a preference model. The key idea is to leverage the structure of the optimal policy under $\pi^*$ as function of the state-action value function $Q^*$ in deterministic MDPs ~\cite{zhou2025q}. This covers the problem of LLM fine tuning as a specific example. To facilitate understanding, we present the relevant results.

For a given parameter $\eta > 0$, the soft-value function $V^{\pi,\eta}$ of a policy $\pi$ is defined as,
\begin{equation}
    V^{\pi,\eta}(s) = \mathbb{E}_{\pi} \left[ \sum_{t=0}^{T-1} r(s_t, a_t) - \eta \, \mathrm{KL}(\pi(s_t) \parallel \pi_{\mathrm{ref}}(s_t)) \Big| s_0 = s\right]
\end{equation}
It can be shown that the KL-regularized RL objective can be solved using the soft Bellman equations. In particular, the optimal policy is given by~\cite{ziebart2010modeling} as
\begin{align}
V_{T}^{\star, \eta}(s) &= 0, \nonumber\\
Q_t^{\star, \eta}(s, a) &= r(s, a) + \mathbb{E}_{s' \sim P(\cdot \mid s,a)}\left[ V_{t+1}^{\star, \eta}(s') \right], \nonumber\\
\pi^{\star, \eta}(a_t \mid s_t) &\propto \pi_{\text{ref}}(a_t \mid s_t) \exp\left( \eta^{-1} Q_t^{\star, \eta}(s_t, a_t) \right), \\
V_t^{\star, \eta}(s) &= \eta \ln \mathbb{E}_{a \sim \pi_{\text{ref}}(\cdot \mid s)} \left[ \exp\left( \eta^{-1} Q_t^{\star, \eta}(s, a) \right) \right] \nonumber.
\end{align}

where $Q_{\star, \eta}$ is the soft-state-action value function under the optimal policy $\pi^*$. In what follows, we specialize our discussion to deterministic transition structure of the LLM generative process. In the sparse reward setting, $V^{\pi,\eta}, Q^{\pi,\eta}$ are functions of the conditional reward distributions of the generations under $\pi_{\mathrm{ref}}$~\cite{zhou2025q}. That is,
\begin{align}
V_{t}^{\star, \eta}(s) &= \eta \ln \mathbb{E}_{\pi_{\text{ref}}} \left[ \exp \left( \eta^{-1}  r(s_{T-1}, a_{T-1}) \right) \middle| s_t = s \right], \\
Q_{t}^{\star, \eta}(s,a) &= \eta \ln \mathbb{E}_{\pi_{\text{ref}}} \left[ \exp \left( \eta^{-1}  r(s_{T-1}, a_{T-1}) \right) \middle| s_t = s, a_t = a \right], \\
\end{align}

\textbf{Preference-based Q Value function:} Our goal is to learn an optimal LLM policy directly using the preference data. 

% \bluetext{
% To begin with, we first derive the soft-state-action value function, and value function in terms of the preference distribution. Formally, from a given context $x$, we define the expected preference of a generation $y \sim \pi(\cdot \mid x)$ over a distribution $\tilde{\pi}$ as
% \begin{equation}
%     \mathcal{P}^*(y \succ \tilde{\pi}) = \mathbb{E}_{y' \sim \tilde{\pi}(\cdot \mid x)}[\mathcal{P}^*(y \succ y' | x)]
% \end{equation}
% where $\mathcal{P}^*(y \succ y' | x)$ is the preference distribution under the BT model of completions $y,y'$ given context $x$. In addition, let $W(y,y' \mid x)$ denote the Bernoulli random variable with mean $\mathcal{P}^*(y \succ y' | x)$. We make the following assumption about the preference distributions .

% \begin{assumption}
% Given a context $x$, the preference distribution of any two pairs of completions are independent of each other. That is, let $(y_1,y'_1)$ and $(y_2,y'_2)$ be 
% \end{assumption}
% \begin{theorem}
%     Under the BT preference model, for any policy $\tilde{\pi}$ we have
%     \begin{align}
%         V_{t}^{\star, \eta}(s) &= \eta \ln \mathbb{E}_{\pi_{\text{ref}}} \left[ \exp \left( \eta^{-1}  \mathcal{P}^*(y \succ \tilde{\pi}) \right) \middle| s_t = s \right], \nonumber \\
% Q_{t}^{\star, \eta}(s,a) &= \eta \ln \mathbb{E}_{\pi_{\text{ref}}} \left[ \exp \left( \eta^{-1} \mathcal{P}^*(y \succ \tilde{\pi}) \right) \middle| s_t = s, a_t = a \right],
%     \end{align}
% \end{theorem}
% \begin{proof}
% Consider the inverse function of the logistic function $\sigma(x)$ given by $\Psi(x) \triangleq \log{\frac{x}{(1-x)}}$. Suppose that the Bradley-Terry model holds, we have
% \begin{align*}
%     \mathbb{E}_{y' \sim \tilde{\pi}(\cdot \mid x)}[\Psi \left(\mathcal{P}^*(y \succ y' | x)\right)] &= \mathbb{E}_{y' \sim \tilde{\pi}(\cdot \mid x)}[\Psi(\sigma(r(y)-r(y')))]\\
%     &= r(y) -  \mathbb{E}_{y' \sim \tilde{\pi}(\cdot \mid x)}[r(y')]\\
%    r(y) &= \mathbb{E}_{y' \sim \tilde{\pi}(\cdot \mid x)}[r(y')] + \mathbb{E}_{y' \sim \tilde{\pi}(\cdot \mid x)}[\Psi \left(\mathcal{P}^*(y \succ y' | x)\right)]
% \end{align*}
% Substituting the reward function into the expressions for optimal  $V_{t}^{\star, \eta},Q_{t}^{\star, \eta}$, the result follows.
% \end{proof}

% Therefore,
% }

To begin with, we first derive the soft-state-action value function, and value function in terms of the preference distribution. For a given context $x$, let $y^{\mathrm{ref}}_x$ be a unique \textit{`reference'} completion starting from state $x$. The preference distribution of any completion $y_x$ given $x$ sampled according to a policy $\pi$ over $y^{\mathrm{ref}}_x$ is given by $\mathcal{P}^*(y_x \succ y^{\mathrm{ref}}_x)$.
% \begin{equation}
%      = \mathbb{E}_{y' \sim \tilde{\pi}(\cdot \mid x)}[\mathcal{P}^*(y \succ y' | x)]
% \end{equation}
% where $\mathcal{P}^*(y \succ y' | x)$ is the preference distribution under the BT model of completions $y,y'$ given context $x$. In addition, let $W(y,y' \mid x)$ denote the Bernoulli random variable with mean $\mathcal{P}^*(y \succ y' | x)$. We make the following assumption about the preference distributions .

% \begin{assumption}
% Given a context $x$, the preference distribution of any two pairs of completions are independent of each other. That is, let $(y_1,y'_1)$ and $(y_2,y'_2)$ be 
% \end{assumption}

% \textcolor{orange}{::Are we treating $\Psi$ as any generic function from some function class or are we treating $\Psi$ as a specific function as used in the proof? We can't use it interchangeably as we have done in the text. Right now it looks more like the former category instead of the latter::}
\begin{theorem}
    Let $\Psi(x) \triangleq \log{\frac{x}{(1-x)}}$. Then, assuming the BT preference model we have
    \begin{align}
        V_{t}^{\star, \eta}(s) &= r(y^{\mathrm{ref}}_s) + \eta \ln \mathbb{E}_{y_s \sim \pi_{\text{ref}}} \left[ \exp \left( \eta^{-1}  \Psi( \mathcal{P}^*(y_s \succ y^{\mathrm{ref}}_s)) \right) \middle| s_t = s \right], \nonumber \\
Q_{t}^{\star, \eta}(s,a) &= r(y^{\mathrm{ref}}_s) + \eta \ln \mathbb{E}_{y_{s'} \sim \pi_{\text{ref}}} \left[ \exp \left( \eta^{-1} \Psi( \mathcal{P}^*(y_{s'} \succ y^{\mathrm{ref}}_s)) \right) \middle| s_t = s, a_t = a \right],
    \end{align}
where $s' = (s | a)$ is the state obtained by concatenating $a$ to state $s$.
\end{theorem}


The above theorem shows that, the expressions $Q_{t}^{\star, \eta}, V_{t}^{\star, \eta}$ are functionals of the preference distribution of completions according to the reference policy $\pi_{\mathrm{ref}}$ with an offset term. The reward function $r^*$ is unknown, however, the optimal policy is a function of the advantage function. Hence, it suffices to evaluate the term with preference distribution. Note that the the reference completion for any given intermediate state $s$ has to be unique. In the rest of the discussion, we choose $y^{\mathrm{ref}}_s$ be the completion obtained by greedy decoding using policy $\pi_{\mathrm{ref}}$


 \textbf{Preference distribution over greedy decoding:} The preference probability $\mathcal{P}^*(y_x \succ y^{\mathrm{ref}}_x)$ can be interpreted as the expected number of 'wins' of a single completion over greedy decoding for a given context.
 Recall that by the virtue of greedy decoding the reference greedy completion $y_x^{\mathrm{ref}}$ is unique. Using the reward-equivalence property of the Bradley Terry model we have the following lemma.

 \begin{lemma}
     Let $r^*$ be the implicit reward function. Then for any given context $x$ and policy $\pi$, there exists a reward function $\tilde{r}$ such that the preference probability of generations $y_x \sim \pi$ over greedy completion is given by $\sigma(\tilde{r}(y))$.
 \end{lemma}

The above lemma plays a crucial role in the development of our algorithm. The above lemma states that the preference probability is solely a function of the completion and the context.One can therefore use a neural network to parameterize $\mathcal{P}^{\theta}(y_x)$, which estimates the expected wins $\mathcal{P}^*(y_x \succ y^{\mathrm{ref}}_x)$ over the greedy completion. From the expression for the optimal policy for the soft-bellman equations, we have
\begin{equation}
\pi^{\star, \eta}(a \mid s) \propto \pi_{\text{ref}}(a \mid s)  \mathbb{E}_{y_{s'} \sim \pi_{\text{ref}}} \left[ \exp \left( \eta^{-1} \Psi( \mathcal{P}^*(y_{s'} \succ y^{\mathrm{ref}}_s)) \right) \middle| s_t = s, a_t = a \right]
\end{equation}
This naturally motivates us to consider parametrized policies of the form $\pi^{\theta}$ such as
\begin{equation}
\pi^{\theta, \eta}(a \mid s) \propto \pi_{\text{ref}}(a \mid s)  \mathbb{E}_{y_{s'} \sim \pi_{\text{ref}}} \left[ \exp \left( \eta^{-1} \Psi( \mathcal{P}^{\theta}(y_{s'} \succ y^{\mathrm{ref}}_s)) \right) \middle| s_t = s, a_t = a \right]
\end{equation}
where $s' = (s | a)$ is the state obtained by concatenating $s$ with action $a$.

 % \textcolor{orange}{::This is very unclear, if $W^*$ is a distribution function, $y$ should be an input. ::}Let $W^*$ denote the conditional distribution of wins of generations from $\pi_{\mathrm{ref}}$. That is,
% \begin{equation}
%     W^*(x \triangleq (s,a) ) \overset{D}{=} \mathrm{Ber}(\cP^*(y \succ y^{\mathrm{ref}}_s | x))
% \end{equation}

% % \bluetext{
% % \begin{enumerate}
% %     \item alternative choice for $P^*(y \succ y^*_s | x)$ is a parametric class where,
% %     $P^*(y \succ y^*_s | x) = \sigma ( \langle \Phi(x),\theta^* \rangle )$. Although, this is what happens in practice we do not have access to $y^*_s$
% % \end{enumerate}
% % }

% where $y$ is a random trajectory under $\pi_{\mathrm{ref}}$, and $y^{\mathrm{ref}}_s$ under the greedy decoding under $\pi_{\mathrm{ref}}$ respectively, starting from state $s$. Therefore, the optimal policy is given by

% \begin{equation}
%     \pi^{\star, \eta}(a \mid s) \propto \pi^{\mathrm{ref}}(a \mid s) \mathbb{E}_{w \sim W^{\star}(s, a)} \left[ \exp\left( \eta^{-1} \Psi(w) \right) \right].
% \end{equation}
% The above expression for the optimal policies leads to distributional learning techniques to estimate the best distribution $\hat{W} \approx W^*$ using maximum likelihood estimation by considering policies of the form $W : \cX \rightarrow \Delta([0,1])$ as 
% \begin{equation}
%     \pi^{W, \eta}(a \mid s) \propto \pi^{\mathrm{ref}}(a \mid s) \mathbb{E}_{w \sim W(s, a)} \left[ \exp\left( \eta^{-1} \Psi(w) \right) \right].
% \end{equation}
% In particular, we consider a parametric class of distributions which closely resembles applications to LLMs.
% \begin{assumption}
% There exists a finite-dimensional vector $\theta^* \in \R^d$ such that 
% \begin{equation}
%      W^*(x \triangleq (s,a) ) \overset{D}{=} \sigma(\langle \Phi(x), \theta^* \rangle)
% \end{equation}
% where $\Phi: \cX \rightarrow \R^d$ is a known embedding function, and $\sigma$ is the logistic function.
% \end{assumption}

\subsection{Algorithm}
In this section we present PITA, a preference guided inference time alignment algorithm for solving the KL-regularized RLHF objective. PITA is an iterative algorithm where progressively better policies are learned by virtue of a parametrized preference function. We describe the PITA algorithm in the context of applications to LLMs; in subsequent section, we provide theoretical convergence results under linear reward approximation.

% Note that the optimal policy is obtained by guided generations of $\pi_{\mathrm{ref}}$ using the regularized  soft-action value function $Q^*$. However, in practice it is difficult to evaluate $Q^*$ unless the distribution on the preference functions for each generation under $\pi_{\mathrm{ref}}$ is known apriori. Assuming a parametric class, one can then use distributional techniques e.g., maximum likelihood for parameter estimation. Moreover, it is unclear if the expectation can be evaluated in closed for beyond simple but restrictive class like Bernoulli~\cite{zhou2025q}. To address this issue, we use certainty equivalence as an approximation for our practical implementation.

Note that the optimal policy is obtained by guiding generations from the reference policy $\pi_{\mathrm{ref}}$ using the regularized soft action-value function $Q^*$. However, in practice, evaluating $Q^*$ is challenging unless the distribution over preference functions for each generation under $\pi_{\mathrm{ref}}$ is known \textit{a priori}. Assuming a parametric family, one can apply distributional techniques---such as maximum likelihood estimation---for parameter inference. Nevertheless, it remains unclear whether the expectation can be computed in closed form beyond simple yet restrictive classes, such as the Bernoulli distribution~\cite{zhou2025q}. To address this, we adopt certainty equivalence as an approximation in our practical implementation.


Let $\hat{\cP}^{\theta}: \cX \rightarrow \Delta([0,1])$ be the preference function that maps a given state $x := (s,a) \in \cX$ to the expected preference under $\pi_{\mathrm{ref}}$, i.e. $\E_{y_x \sim \pi_{ref}}[\cP^*(y_x \succ y^{\mathrm{ref}}_s)]$. Then the natural loss is the binary cross-entropy loss (BCE), i.e.,
\begin{equation}
    \mathcal{L}(o_y,\hat{\cP}) = - o_y \log{\hat{\cP}} - (1 - o_y) \log{( 1 - \hat{\cP})}
\end{equation}
where $o_y = \mathbf{1}_{y \succ y^{\mathrm{ref}}}$ is the indicator function of the completion $y$ preferred over the reference completion $y^{\mathrm{ref}}$.

The algorithm iteratively updates the estimator parameters $\theta$ using new preference information collected by the induced policy $\pi_k \triangleq \pi^{\theta_k,\eta}$. In particular, the data collection strategy follows a rollout step using $\pi^{k}$ for $t$ steps until a context $s_t$ is sampled. Then, a completion is randomly sampled starting from this context along with greedy decoding using $\pi_{ref}$. The preference as observed between the two completions is precisely a sample from $\cP^*$. These preference samples are added to the dataset, and parameters are updated via gradient descent. The procedure is repeated until convergence. The pseudocode for the algorithm is detailed in Algorithm~\ref{alg:PITA}

\begin{algorithm}[H]
\caption{Preference Guided Inference Time Alignment (PITA)}
\label{alg:PITA}
\begin{algorithmic}[1]
\State \textbf{Input:} reference policy $\pi^{\text{ref}}$. Initialize $\theta_0$ and dataset $\mathcal{D} = \emptyset$
\For{$k = 1, 2, \dots$ until convergence}
    \State Let $\pi^{k-1} \leftarrow \pi^{{\theta_{k-1}},\eta}$ be policy induced by $\hat{\cP}^{\theta_{k-1}}$.
    \For{$i = 1, 2, \dots, N$}
        \State Sample a roll out step uniformly  $t \sim \mathrm{Unif}([T])$.
        \State Roll in with $\pi^{k-1}$ for $t$ steps to get the context $s_{t}$.
        \State Sample the  reference response $y^{\mathrm{ref}}_{s_{t}}$ starting from context $s_{t}$ using greedy decoding.
        \State Sample M responses $y_{s_t}^1,\cdots, y_{s_t}^M$ with $\pi^{\text{ref}}$ starting from $s_t$.
        \State Add $(s_t,y_{s_t}^i,y^{\mathrm{ref}}_{s_{t}}, \mathbf{1}_{y_i \succ y^{\mathrm{ref}}_{s_{t}}})$ to  $\mathcal{D}$, $\forall i \in [M]$.
    \EndFor
    \State Update $\theta^k$ by Maximum Likelihood Estimation on the aggregated data:
    \[
    \theta^{k} \leftarrow \arg\min_{\theta}  \E_{(x,y,y') \sim \cD} \left[ \mathcal{L}(\mathbf{1}_{y \succ y'},\hat{\cP}^{\theta}) \right]
    \]
\EndFor
\State \textbf{Output:} Final $\theta^k$.
\end{algorithmic}
\end{algorithm}

 We remark that our algorithm belongs to the class of value-based algorithms for post-training LLM\cite{mudgal2023controlled,han2024value,zhou2025q}. In CD~\cite{mudgal2023controlled} and VAS~\cite{han2024value}, the learned Q-function is a non-regularized version of the optimal $Q^*$. In contrast, Q-sharp~\cite{zhou2025q} aims to learn the optimal state-action value function using distributional reinforcement learning~\cite{bellemare2023distributional}.
Our iterative algorithm shares design principles with Q-sharp; however, it learns the optimal action-value function directly from preference data, eliminating the need for a pre-trained model.





==> arxiv/sections/OLD-theory.tex <==
\section{Theoretical Results}

In this section, we show theoretical guarantees for the special case of linear reward class.

\begin{assumption}\label{assum:theta_bound}
The reward lies in the family of linear functions $r_{\theta}(y) = \theta^\top \Phi(y)$ for some known $\Phi$ with $\sup \|\Phi(\cdot)\|_2 \leq L$. Let $\theta^\star$ be the true parameter. To ensure the identifiability of $\theta^\star$, we let $\theta^\star \in \Theta_B$, where
\[
\Theta_B = \left\{ \theta \in \mathbb{R}^d \mid \langle \mathbf{1}, \theta \rangle = 0, \|\theta\|_2 \leq B \right\}.
\]
\end{assumption}

\subsection{Preference Modeling in PITA}
We denote by $\Phi(x)$ the $d$-dimensional embedding of a state $x$ where $\Phi : \cX \rightarrow \R^d$. The embedding function is known to the learner. In the context of LLMs, such a $\Phi$ is obtained by the hidden representation of the last but second layer of the model. The set of all completions starting from a given state $x$ are denote by $\cY^{\pi}_x = \left\{y: y \sim \pi(\cdot |x)\right\}$. Thus the preference distribution $\cP^*(y_x)$ for a completion $y_x \in \cY^{\pi}_x$ is given by
\begin{equation}
    \cP^*(y_x) = \cP^*(y_x \succ y_x^{\pi}) = \sigma(\langle \theta^*, \Phi(y_x) \rangle - \langle \theta^*, \Phi(y_x^{\pi}) \rangle)
\end{equation}
where $y_x^{\pi}$ is the greedy completion under $\pi$. Using the fact that the greedy completion is unique given a starting state/context $x$ for a fixed policy $\pi$. With slight abuse of notation, for PITA, we have a parametric class of preference distributions given by
\begin{equation}
    \cP^{\theta}(y_x) = \sigma(\langle \theta, \Phi(y_x) - \Phi(y_x^{\pi_{\mathrm{ref}}}) \rangle) 
\end{equation}
Now, since $y_x^{\pi_{\mathrm{ref}}}$ is fixed, we can, without loss of generality we can renormalize $\Phi(y_x^{\pi_{\mathrm{ref}}})$ to $0$ since all preference data given $x$ is measured with respect to $y_x^{\pi_{\mathrm{ref}}}$. Hence,
\begin{equation}
    \cP^{\theta}(y_x) = \sigma(\langle \theta, \Phi(y_x) \rangle)
\end{equation}
Here $\theta \in \Theta_B$, and $y_x \in \cY^{\pi_{\mathrm{ref}}}_x$. In what follows, we drop the context $x$ from our notation as the results can be applied on a per-context basis.

\textbf{Maximum Likelihood Estimation (MLE)}
In the above preference modeling, a natural way to compute an estimator $\theta_k$ given completion pairs $\{(x_i,y_i,y^{\mathrm{ref}}_i)\}_{i=1}^n$, and their preference feedback values $\{o_i\}_{i=1}^n$ is maximum likelihood estimation . MLE minimizes the negative log-likelihood function, defined as:
\begin{align}
\hat{\theta} &\in \arg \min_{\theta \in \Theta_B} \mathcal{L}_{\mathcal{D}}(\theta), \\
\mathcal{L}_{\mathcal{D}}(\theta)
&= - \sum_{i=1}^n o_i \log{\sigma(\langle \theta, \Phi(y_i) \rangle)} + 
(1 - o_i) \cdot \log{1 - \sigma(\langle \theta, \Phi(y_i) \rangle)}.
\end{align}

Following results from dueling bandits, and reinforcement learning~\cite{faury2020improved,shah2016estimation,pacchiano2021dueling}, we have convergence of MLE to the true parameter.
\begin{lemma}\label{eqn:mle}
Under Assumption~\ref{assum:theta_bound}, for any $\lambda > 0$, with probability at least $1 - \delta$ we have
\begin{equation}
\left\|\hat{\theta} - \theta^*\right\|_{\Sigma_{\mathcal{D}} + \lambda I} \leq C \cdot \sqrt{\frac{d + \log(1/\delta)}{\gamma^2 n} + \lambda B^2} .
\end{equation}

where $\Sigma_{\mathcal{D}} = \frac{1}{n} \sum_{i=1}^n \Phi(y_i) \Phi(y_i)^\top$, 
$\gamma = \frac{1}{2 + \exp(-LB) + \exp(LB)}$.
\end{lemma}

\subsection{Regret}
We now state our main PAC result on PITA. We make the following assumption on the boundedness of the embedding function.

\begin{assumption}\label{assum:emb-norm-bound}
(The single concentrability coefficient)~~Consider the space of all policies of the form 
$\Pi_{\theta} \triangleq \{ \pi_{\theta}: \pi_{\theta} \propto \pi_{\mathrm{ref}} \exp{(\eta^{-1} \Phi)} \}$.
We assume $\left\|(\Sigma_{\mathcal{D}} + \lambda I)^{-1/2} \mathbb{E}_{y \sim \pi} [\Phi(y)] \right\|_2$ is bounded for all $\pi \in \Pi_{\theta}$. 
\end{assumption}

\begin{theorem}
For any $\lambda > 0$, with probability at least $1 - \delta$,
\begin{equation}
\sum_{k=1}^K (V^{\star,\eta} - V^{\theta_k,\eta}) \leq C \sum_{k=1}^K  \cdot \left( \sqrt{\frac{d + \log(1/\delta)}{\gamma^2 n_k} + \lambda B^2}  \cdot \sup \left\|(\Sigma_{\mathcal{D}} + \lambda I)^{-1/2} \mathbb{E}_{y \sim \pi} [\Phi(y)] \right\|_2 \right).
\end{equation}
where $n_k$ is the number of preference samples collected upto iteration $k$, and $\pi \in \Pi_{\theta}$.
\end{theorem}


==> arxiv/sections/app-d-experiments-v2.tex <==

\section{Implementation Details and Sentiment Generation}\label{app:experiments}
In this section we describe training details for PITA on GSM8K, and star graph reasoning. Additionally, we present our results in detail for sentiment generation tasks~\cite{chaudhary2025riskaversefinetuninglargelanguage}

% \subsection{Datasets and Models}\label{app:datasets}

\subsection{Math Reasoning}\label{app:math}
\paragraph{Dataset.}  \textbf{GSM8K} contains \(7{,}500\) training and \(1{,}319\) test problems.  
We create a \(90\%/10\%\) split of the original training set for learning and validation, reserving the full test set for final reporting.

\paragraph{Models.}  We use the \textbf{Llama-3 8B-Instruct} model as our reference policy and the \textbf{Llama-3.2 1B-Instruct} model ~\cite{grattafiori2024llama} as the backbone for our Value function estimation. For Q\#-HF, the reward model trained from preference data is also a Llama-3.2 1B-Instruct. We use the OpenMathInstruct-2 model~\cite{toshniwal2024openmathinstruct} for preference data generation between two pairs of responses for it's reasonably high accuracy on arithmetic reasoning tasks such as GSM8K.

% \paragraph{Algorithms.}  We evaluate the following approaches against the base reference model \(\pi_{\text{ref}}\):

% \begin{itemize}[leftmargin=1.4em]
%     \item \textbf{Q\#}:  The algorithm described in ~\cite{zhou2025q} trained directly on the GSM8K dataset with access to the true binary reward labels.  
%     \item \textbf{Q\#-HF}:  A {\em two-stage} procedure: first, a reward model is trained from GSM8K preference pairs; this learned reward is then used in the Q\# algorithm to obtain the final policy.  
%     \item \textbf{PITA (ours)}:  The algorithm described in Section~4, which learns a soft \(Q\)-function directly from preference data and induces the final policy without requiring a reward model from preference data.  
% \end{itemize}

% \paragraph{Training hardware.}   
% All training and evaluation are performed on a single NVIDIA A100 80 GB GPU. 

\textbf{Training details.} We collect pairwise samples for each question in the training set of GSM8K and label every sample either as \textit{'preferred'} (1) or \textit{'not preferred'} (0) based on the quality of final answer. Note that for arithmetic reasoning, there is an exact numeric answer for each question. A correct answer is automatically preferred over a wrong answer. If the samples from a given pair are either both correct, or both wrong a preference is assigned based by the OpenMathInstruct-2 model.
% PITA trains for 10 policy-evaluation/optimization cycles ( 5 per round), each with a learning rate of $2 \times 10^{-5}$ and a context length of 4096. 
% The model is trained from scratch between rounds where each round uses training data collected from previous rounds in addition to the current one.
% The baseline uses identical hyperparameters. Each optimization run uses a single NVIDIA A100 GPU. 
PITA is trained over 10 policy evaluation/optimization cycles (5 per round), using a learning rate of $2 \times 10^{-5}$ and a context length of 4096. The model is retrained from scratch at the start of each round, using data collected from both the current and all previous rounds. The baseline model is trained with identical hyperparameters. Each optimization run is performed on a single NVIDIA A100 GPU.

\paragraph{Evaluation protocol.}  
We report single-sample accuracy (\textit{pass@1}) and majority-vote accuracy over \(k{=}\!8\) samples (\textit{maj1@8}).  
Generations use temperature \(T=0.8\) and nucleus sampling \(p=0.9\). We use the inference optimizations for value function $V$ given in ~\cite{zhou2025q}. Similar to Q\# we train PITA for two iterations and observe performance converging. All evaluations are done with zero-shot prompting.

The prompt template used for evaluation is:
\texttt{'Problem:\textbackslash n\textbackslash n\{0\} Write your answer inside \textbackslash\textbackslash boxed\{\{\}\}.\textbackslash n\textbackslash nSolution:'}
where \texttt{\{0\}} is replaced by the actual question from the dataset.



% \paragraph{Discussion.}  
% Table~\ref{tab:pita-gsm8k-correct} shows that PITA attains performance on par with Q\# even without access to the true reward labels. Despite using a learned reward model with increased availability of preference data, Q\#-HF fails to perform as well as PITA, highlighting the brittleness of reward estimation in this setting. This suggests that PITA's preference-based approach is more robust and effective in aligning model outputs with desired preferences.

%  Additionally, the KL-Divergence of PITA is higher than that of Q\# and Q\#-HF. This is because the language model used to provide preference feedback in PITA is OpenMathInstruct-2, which is distinct from the rule-based reward function score used in Q\#. This highlights the tradeoff between alignment with the reference policy and the flexibility of preference-based feedback.

% \subsection{Math Reasoning}\label{app:math}

% We benchmark \textbf{PITA} on the GSM8K grade-school arithmetic corpus~\cite{cobbe2021training}.

% \paragraph{Dataset.}  \textbf{GSM8K} contains \(7{,}500\) training and \(1{,}319\) test problems.  
% We create a \(90\%/10\%\) split of the original training set for learning and validation, reserving the full test set for final reporting.

% \paragraph{Models.}  We use the \textbf{Llama-3 8B-Instruct} model as our reference policy and the \textbf{Llama-3.2 1B-Instruct} model ~\cite{grattafiori2024llama} as the backbone for our Value function. For Q\#-HF the reward model trained from preference data is also a LLama-3.2 1B-Intstruct.


% \paragraph{Algorithms.}  We evaluate the following approaches against the base reference model \(\pi_{\text{ref}}\):

% \begin{itemize}[leftmargin=1.4em]
%     \item \textbf{Q\#}:  The algorithm described in ~\cite{zhou2025q} trained directly on GSM8K dataset with access to the true binary reward labels.  
%     \item \textbf{Q\#-HF}:  a {\em two-stage} procedure - first a reward model is trained from GSM8K preference pairs; this learned reward is then plugged into the Q\# algorithm to obtain the final policy.  
%     \item \textbf{PITA (ours)}:  the algorithm mentioned in of Section~4, which learns a soft \(Q\)-function directly from preference data and induces the final policy without having to learn a reward model from preference data.  
% \end{itemize}

% \paragraph{Training hardware.}   
% All training and evaluation are performed on a single NVIDIA A100 80 GB GPU. 

% \paragraph{Evaluation protocol.}  
% We report single-sample accuracy (\textit{pass@1}) and majority-vote accuracy over \(k{=}\!8\) samples (\textit{maj1@8}).  
% Generations use temperature \(T=0.8\) and nucleus sampling \(p=0.9\).

% \begin{table}[H]
%   \centering
%   \caption{GSM8K accuracy (\%) and KL divergence.}
%   \label{tab:pita-gsm8k-correct}
%   \begingroup
%   \setlength{\tabcolsep}{6pt}
%   \renewcommand{\arraystretch}{1.2}
%   \begin{tabular}{lccc}
%     \toprule
%     \textbf{Algorithm} & \textbf{pass@1} & \textbf{maj1@8} & \textbf{KL}↓ \\
%     \midrule
%     $\pi_{\text{ref}}$  & 69.1 & 85.8 & - \\
%     Q\#                 & 78.4 & 88.1 & 2.65 \\
%     Q\#-HF              & 67.23 & 78.09 & 2.48 \\
%     \midrule
%     \textbf{PITA (ours)}& 75.92 & 86.81 & 21.67 \\
%     \bottomrule
%   \end{tabular}
%   \endgroup
% \end{table}

% \textbf{Reward-Model Calibration in Q\#-HF:} Figure~\ref{fig:reward_hist_correct} contrasts reward scores assigned by the BT model to correct versus incorrect generations produced by the baseline. A larger separation indicates stronger alignment between the reward and task success. The reward model here was trained for 10 epochs, whereas the one in ~\ref{fig:reward_hist} was trained for half an epoch. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{neurips2025/figures/histograms/figu-hist-2.pdf}
%     \caption{Distribution of learned reward scores w.r.t preferred/correct (green) and not preferred/incorrect (red) for ID(in-dist.)/OOD(out-of-dist.) data.  The reward function is difficult to learn.}
%     \label{fig:reward_hist_correct}
% \end{figure}


% \paragraph{Discussions.}  
% Table~\ref{tab:pita-gsm8k-correct} shows that PITA attains performance on par with Q\# even without having knowledge of the true reward labels. Q\#-HF despite using a learnt reward model that is well aligned with the true reward signal as demonstrated in ~\ref{fig:reward_hist_correct} fails to perform as well as PITA.



%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Star-Graph Reasoning}
We now describe the training methodology used to apply \textbf{PITA} to the star-graph task.

\textbf{Training Setup:} We follow the experimental setup of Q\#~\cite{zhou2025q} to generate and evaluate the star-graph datasets. All models are initially pretrained using next-token prediction on a dataset of 200k randomly sampled graphs paired with their correct paths.

We consider several baselines, including \textbf{REINFORCE}, \textbf{DPO}, \textbf{RPO}—as well as value-based methods \textbf{Q\#} and \textbf{CD}. Post-training is conducted on a separate dataset of 200k new random graphs. To ensure a fair comparison, we reproduce the results with an identical reward structure and reuse the datasets used in~\cite{zhou2025q}. For REINFORCE, a reward of 1 is assigned for correct paths and \(-0.1\) for incorrect ones. For DPO and RPO, pairwise comparisons between a correct path \(y_{\text{chosen}}\) and an incorrect shortcut path \(y_{\text{reject}}\) are sampled from the pre-trained model. Similarly, for \textbf{Q\#}, a classifier is trained on the same pairwise dataset, labeling correct paths with reward 1 and incorrect ones with 0. Note that PITA uses a unique reference generation at the core of its algorithm. In PITA, we treat correct paths as the \textit{`preferred'} solution and the incorrect path as the \textit{`not-preferred'} answer to estimate the preference distribution. The unique correct answer naturally serves as the reference completion for the star-graph task. 

All models are trained for 10 epochs using the AdamW optimizer with a weight decay of $0.1$ and a batch size of $256$. The learning rates are set to $2.5 \times 10^{-4}$ for pretraining, $1 \times 10^{-5}$ for REINFORCE, and $1 \times 10^{-4}$ for DPO, RPO, CD, and Q\#. For Q\# and CD, we set the inverse temperature parameter $\eta = 0.1$. Training is performed on a single A100 GPU. Evaluation is conducted on a held-out test set of 20k graphs using top-$k = 10$ sampling and temperature $1.0$.

% \paragraph{Discussion.}  
% The star-graph experiments provide valuable insights into why PITA outperforms standard policy-based methods, as well as other value-based algorithms like Q\# and CD. While REINFORCE achieves a maximum accuracy of \(1/d\), the performance of DPO is significantly worse. We observe similar behavior to that reported in~\cite{zhou2025q}, where DPO achieves \(0\) accuracy, with the policy collapsing probabilities to \(0\). In contrast, value-based methods perform better across all graph configurations. Notably, PITA achieves further performance improvements, even when baseline reward-based methods are already near perfect accuracy. This improvement in accuracy can be attributed to PITA's ability to generate more precise implicit rewards. Upon examining the rewards generated by Q\# for the star-graph reasoning test set, we find that the reward differences between correct and incorrect answers are significantly smaller compared to those generated by PITA.


% The star-graph experiments provide insight into why PITA is effective compared to standard policy-based methods, and even other value-based algorithms like Q\# and CD. While REINFORCE has an accuracy of at most \(1/d\), the performance of DPO is lacking. We observe similar behavior as reported in~\cite{zhou2025q} with \(0\) accuracy for DPO, where the policy collapses the probabilities to \(0\). In contrast, the value-based methods achieve better performance across all graph configurations. In particular, we would like to highlight the performance gains of PITA, even though it is already close to perfect accuracy with baselines based on reward-based methods. The increase in accuracy is due to finer implicit reward generation by PITA. Taking a closer look at the rewards generated by Q\# for the star-graph reasoning task test set, we observe that the difference in rewards assigned between correct and incorrect answers is significantly lower compared to what PITA generates.




% In this section, we demonstrate the effectiveness of \textbf{PITA} in guiding a reference language model (LM) to achieve near-perfect generalization accuracy on the star-graph task~\cite{bachmann2024pitfalls}, outperforming value-based baselines such as \textbf{Q\#}~\cite{zhou2025q} and \textbf{CD}~\cite{mudgal2023controlled}. A star-graph $\mathcal{G}(d, l)$ is defined as a tree with $d$ paths of length $l$ emanating from a common root node. The goal is for the LM to generate the correct path from the root to a leaf, given the edge set defining the graph. Figure~\ref{fig:star-graph} illustrates the star-graph task.

% \begin{figure}[H]
%   \centering
%   \includegraphics[width=\textwidth]{neurips2025/figures/star-graph.pdf} % replace with your filename
%   \caption{A $\cG= (3,8)$ star-graph configuration with degree $d=3$, and path length $l=8$. Pre-trained model with next-token prediction, learns a faulty shortcut which selects a random first node, and follow the path from there on.}
%   \label{fig:star-graph}
%   \vspace{-0.2in}
% \end{figure}

% Despite the task’s structural simplicity, \cite{bachmann2024pitfalls} highlight a key failure mode in models trained with next-token prediction. Specifically, the model often learns a \textit{Clever-Hans} shortcut—selecting the first node in the root’s adjacency list and following it to a leaf. While this heuristic yields perfect accuracy on the training set, it fails to generalize: on unseen test graphs, the model selects the correct path only with probability $1/d$, since the first adjacent node is correct only $1/d$ of the time.

% Zhou et al.~\cite{zhou2025q} show that such faulty behavior can be corrected during post-training using value-based methods. However, widely used policy-based approaches like REINFORCE~\cite{ahmadian2024back}, DPO~\cite{rafailov2023direct}, and RPO~\cite{pang2024iterative} are unable to overcome this shortcut, achieving test accuracy no better than $1/d$. This failure is likely due to the difficulty transformer-based architectures face when unlearning spurious heuristics via policy-gradient optimization~\cite{hu2024learning}.

% We now describe the training methodology used to apply \textbf{PITA} to the star-graph task.

% \textbf{Training Setup:} We closely follow the experimental setup of Q\#~\cite{zhou2025q} to generate and evaluate the star-graph datasets. We report test accuracies of PITA(ours) on three classes of graphs smaller graphs $\mathcal{G}(2, 5)$ and $\mathcal{G}(5, 5)$, where we employ the GPT-2 small model, and a larger graph $\mathcal{G}(3, 8)$, for which we use the GPT-2 medium model~\cite{radford2019language} to train the set of \textit{pre-trained models}.
% All models are initially pretrained using next-token prediction on a dataset of 200k randomly sampled graphs paired with their correct paths. 

% We consider several baselines which include \textbf{REINFORCE},\textbf{DPO},\textbf{RPO}—as well as value-based methods \textbf{Q\#} and \textbf{CD}. Post-training is conducted on a separate dataset of 200k new random graphs.
% In order to have a fair comparison, we reproduce the results with identical reward structure, and reuse the datasets used in~\cite{zhou2025q}.
% For REINFORCE, a reward of $1$ is assigned for correct paths and $-0.1$ for incorrect ones.
% For DPO and RPO, pairwise comparisons between a correct path $y_{\text{chosen}}$ and an incorrect shortcut path $y_{\text{reject}}$ are sampled from the pre-trained model. Similarly, for \textbf{Q\#}, a classifier is trained on the same pairwise dataset, labeling correct paths with reward $1$ and incorrect ones with $0$. Note that PITA uses a unique reference generation at the core of it's algorithm.
% In PITA, we treat correct paths as the \textit{`preferred'} solution and the incorrect path as the \textit{`not-preferred'} answer to estimate the preference distribution. The unique correct answer naturally serves as the reference completion for the star-graph task.
% We report our test results in Table~\ref{tab:pita-star-graph}

% \begin{table}[H]
%     \centering
%     \caption{Comparison of PITA with other baselines across star-graph configurations.}
%     \label{tab:pita-star-graph}
%     \begingroup
%     \setlength{\tabcolsep}{6pt}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lccc}
%         \toprule
%         \textbf{Algorithm} & $\mathcal{G}(2,5)$ & $\mathcal{G}(5,5)$ & $\mathcal{G}(3,8)$ \\
%         \midrule
%         pre-trained & 49.94 & 19.8 & 33.24 \\
%         Q\# & 99.90 & 97 & 98.62 \\
%         CD & 99.94 & 98.62 & 99.52 \\
%         REINFORCE & 49.19 & 13.13 & 25.96 \\
%         DPO & 37.61 & 0.0 & 0.0 \\
%         RPO & 49.69 & 19.93 & 33.47 \\
%         \midrule
%         \textbf{PITA (ours)} & 99.97 & 99.7 & 99.93 \\
%         \bottomrule
%     \end{tabular}
%     \endgroup
% \end{table}


% All models are trained for 10 epochs using the AdamW optimizer with a weight decay of $0.1$ and a batch size of $256$. The learning rates are set to $2.5 \times 10^{-4}$ for pretraining, $1 \times 10^{-5}$ for REINFORCE, and $1 \times 10^{-4}$ for DPO, RPO, CD, and Q\#. For Q\# and CD, we set the inverse temperature parameter $\eta = 0.1$. Training is performed on a single A100 GPU. Evaluation is conducted on a held-out test set of 20k graphs using top-$k = 10$ sampling and temperature $1.0$.

% \textbf{Discussion.}
% The star-graph experiments provides us insight into why PITA is effective compared to the standard policy based methods, and even the other value based algorithms like $Q\#$ and CD. While REINFORCE has an accuracy of at most $1/d$, the performance of DPO is lacking. We observe a similar behavior as reported in~\cite{zhou2025q} with $0$ accuracy for DPO where the policy collapses the probabilities to 0. In contrast the value based methods achieve better performance across all graph configurations. In particular, we would like to highlight the performance gains of PITA despite already close to perfect accuracy with baselines based on reward based methods. We notice that the increase in accuracy is due to finer implicit reward generation by PITA. Taking a closer look at the rewards generated by $Q\#$ for the star graph reasoning task test set, the difference of rewards assigned between correct and incorrect answers are significantly lower compared to what PITA gives.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{IMDB Sentiment Generation}\label{app:imdb}

In this section we evaluate \textbf{PITA} on controlled sentiment generation. The task follows the IMDB-Gen setting of ~\cite{ramamurthy2023reinforcementlearningnotnatural} and ~\cite{chaudhary2025riskaversefinetuninglargelanguage}. Given the first 60 tokens of a movie review, the language model must continue the text so that the completed review expresses maximally positive sentiment.

\paragraph{Dataset.} We use the \textbf{IMDB Reviews} dataset, which contains \(25{,}000\) training and \(25{,}000\) test reviews, each labeled \emph{positive} or \emph{negative}. For each example, we truncate the review to its first 60 tokens, which form the prompt \(x\); the model then generates up to 60 continuation tokens \(y\). The reward model for this task is the \textbf{lvwerra/distilbert-imdb} classifier, with the logit corresponding to the positive sentiment output node used as the scalar reward. For the creation of the preference dataset, we select the generation with the higher reward as the preferred generation.

\paragraph{Models.} For this task, we use \textbf{TinyLlama-1.1B-Chat}\footnote{\url{https://huggingface.co/TinyLlama/TinyLlama-1.1B-Chat}} as both our reference policy and the backbone for our value function. For the reward model learned from the preference data for Q\#-HF, we use a \textbf{LLama 3.2 1B-Instruct} model.

\paragraph{Evaluation} We evaluate the same set of algorithms as above. For each of the \(5{,}000\) \textbf{IMDB} test set prompts, we sample a \emph{single} continuation using nucleus sampling with top-\(p = 0.9\) and temperature \(T = 0.8\). The full prompt + completion is scored by the \texttt{lvwerra/distilbert-imdb} sentiment classifier. We report the mean sentiment logit score (\textsc{Sent.}↑) and the token-level KL divergence (\textsc{KL}↓) between the fine-tuned policy and the reference model \(\pi_{\text{ref}}\).  An example of the completions generated by $\pi_{\text{ref}}$ and by PITA is shown in Figure~\ref{fig:imdb_example}.

\begin{table}[H]
  \centering
  \caption{IMDB-Gen: sentiment (higher is better) and KL divergence (lower is better) on 5,000 test prompts.}
  \label{tab:pita-imdb}
  \begingroup
  \setlength{\tabcolsep}{8pt}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{lcc}
    \toprule
    \textbf{Algorithm} & \textsc{Sent.}↑ & \textsc{KL}↓ \\
    \midrule
    $\pi_{\text{ref}}$ & -0.52 & - \\
    Q\#                & 0.22 & 7.51 \\
    Q\#-HF             & -0.44 & 5.22 \\
    \midrule
    \textbf{PITA (ours)} & 0.01 & 7.27 \\
    \bottomrule
  \end{tabular}
  \endgroup
\end{table}

\paragraph{Discussion.} The range of rewards generated by \texttt{lvwerra/distilbert-imdb} typically lies between -3 and +3. Q\# with access to true rewards performs the best. Among the algorithms that only have access to a preference signal, rather than the true reward, PITA performs the best. 

Sentiment alignment is inherently difficult, and Q\# has access to a pre-trained DistilBERT model specifically tuned for sentiment analysis. In contrast, reproducing a preference function with a similar structure requires much more preference data. Despite this challenge, PITA is able to extract valuable information from the given preference data and significantly outperforms Q\#-HF, which appears to have poorly learned a reward model. This demonstrates PITA's ability to leverage limited preference data for effective alignment.



%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%

% \subsection{IMDB Sentiment Generation}\label{app:imdb}

% We next evaluate \textbf{PITA} on controlled sentiment generation.  The task follows the IMDB-Gen setting of ~\cite{ramamurthy2023reinforcementlearningnotnatural} and ~\cite{chaudhary2025riskaversefinetuninglargelanguage}. Given the first 60 tokens of a movie review, the language model must continue the text so that the completed review expresses maximally positive sentiment.

% \paragraph{Dataset.}
% We use the \textbf{IMDB Reviews} dataset that contains \(25{,}000\) training and \(25{,}000\) test reviews, each labelled \emph{positive} or \emph{negative}.  
% For every example we truncate the review to its first 60 tokens, which form the prompt \(x\); the model then generates up to 60 continuation tokens \(y\).  The reward model for this task is the \textbf{lvwerra/distilbert-imdb} classifier. We use the logit corresponding to the positive sentiment output node as the scalar reward. For the creation of a preference dataset we simply choose the generation with a higher reward as the preferred generation.  

% \paragraph{Models.}
% For this task we use \textbf{TinyLlama-1.1B-Chat} \footnote{\url{https://huggingface.co/TinyLlama/TinyLlama-1.1B-Chat}} as both our reference policy and the backbone for our value function.  
% For the reward model learnt from the preference data for Q\#-HF we use a \textbf{LLama 3.2 1B-Instruct} model.



% \paragraph{Evaluation}
% We evaluate the same set of algorithms as above. For each of the \(5{,}000\) \textbf{IMDB} test set prompts we sample a \emph{single} continuation using nucleus sampling with top-\(p = 0.9\) and temperature \(T = 0.8\).  
% The full prompt + completion is scored by the \texttt{lvwerra/distilbert-imdb} sentiment classifier.  
% We report the mean sentiment logit score (\textsc{Sent.}↑) and the token-level KL divergence (\textsc{KL}↓) between the fine-tuned policy and the reference model \(\pi_{\text{ref}}\).

% \begin{table}[H]
%   \centering
%   \caption{IMDB-Gen: sentiment (higher is better) and KL divergence (lower is better) on 5 000 test prompts.}
%   \label{tab:pita-imdb}
%   \begingroup
%   \setlength{\tabcolsep}{8pt}
%   \renewcommand{\arraystretch}{1.2}
%   \begin{tabular}{lcc}
%     \toprule
%     \textbf{Algorithm} & \textsc{Sent.}↑ & \textsc{KL}↓ \\
%     \midrule
%     $\pi_{\text{ref}}$ & -0.52 & - \\
%     Q\#                & 0.22 & 7.51 \\
%     Q\#-HF             & -0.44 & 5.22 \\
%     \midrule
%     \textbf{PITA (ours)} & 0.01 & 7.27 \\
%     \bottomrule
%   \end{tabular}
%   \endgroup
% \end{table}

% \paragraph{Discussion.} The range of rewards generated by \texttt{lvwerra/distilbert-imdb} typically lies between -3 to +3. Q\# with access to true rewards performs the best. Among the algorithms that only have access to a preference signal as opposed to the true reward PITA performs the best. 

% We attribute the inability of PITA to perform as well as Q\# in this task to the lack of preference data compared to math reasoning task. (Here we have 5 )

\begin{figure}[ht]
\centering
\begin{minipage}{\textwidth}
\begin{tcolorbox}[colback=white, colframe=black]

\textbf{Prompt:} Paul Mazursky misfires on this film. The writing, direction, casting, and acting (with the exception of Victorio Gassman) are all off the mark. I remember the reviews from 20+ years ago being mediocre, but I thought it still might

\dasheddline

\textbf{Completion from $\pi^{\text{ref}}$:} \textcolor{red!80!black}{be good. But by today's standards, the film just isn't good enough. It's a muddled and overly long (about 2 1/2 hours) film that ultimately does not live up to its potential as a classic film noir.
}\\ 
\dasheddline

\textbf{Completion from PITA:} \textcolor{blue!30!green}{be good. I'm glad to see how far it's come. This is not a great film, but it's definitely a lot better than the original. I think that makes it more enjoyable to watch. The acting is excellent, with a lot of great performances by both Mar
}





\end{tcolorbox}
\end{minipage}
\caption{Comparison of IMDB review completions (constrained to 60 tokens) from $\pi_{\text{ref}}$ vs PITA.  PITA is able to change the sentiment positive, while $\pi_{\text{ref}}$ fails to do so.}  % involving book fractions.}
\label{fig:imdb_example}
\end{figure}


\section{Additional Experimental Details}\label{app:additonal-experiments}





\subsection{Ablation Study on PITA training for GSM8K}

We benchmark \textbf{PITA} on the GSM8K grade-school arithmetic corpus~\cite{cobbe2021training}, which was also considered in the main paper. In contrast to the main paper, we evaluate PITA with only a single round of training i.e. ($k=1$ in Algorithm 1). We present our results in Table~\ref{tab:gsm8k_app_ablation}



\begin{table}[H]
    \centering
    \caption{Performance on the \textsc{GSM8K} \emph{test} split.}
    \label{tab:gsm8k_app_ablation}
    \begingroup
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Algorithm} & \textbf{pass@1} $\uparrow$ & \textbf{maj@8} $\uparrow$ & \textbf{KL}  \\
        \midrule
        $\pi_{\mathrm{ref}}$ & 69 & 85 & - \\
        Q\# & 78.4 & 88.1 & 2.65 \\
        Q\#-HF & 49.9 & 72.0 & 18.85 \\
        \midrule
        PITA (ours)  & 74.8 & 86.1 & 18.4 \\
        \bottomrule
    \end{tabular}
    \endgroup
\end{table}

We see a clear drop in performance when trained with limited data in both pass@1, and maj@8 metrics. Although the choice of two rounds ($k=2$ in Algorithm 1) was made to achieve a fairer comparison with Q\#, an additional round  of training allows for a greater diversity of preference data. The iterative training process is a key step in enabling PITA to better adapt to the preferences, leading to more robust results in alignment tasks.

\subsection{Reward Training for Q#-HF}

Recall that Q\#-HF trains a reward model as an intermediate step for using the Q\# algorithm. We would like to highlight the sensitivity of algorithmic performance of reward training methods.
The results from Table~\ref{tab:gsm8k_app_ablation} involve a single round of training. That is, to ensure a fair comparison with other algorithms, the reward function for single-round Q\#-HF was trained using only 50\% of the data used in the main paper, so that the total data across reward estimation and policy training remained comparable. We observe a substantial drop in performance of the Q\# baseline which can we attributed to the poor reward separation between correct and incorrect generations as shown below.

% Given that Q\#-HF performed poorly in this setup, we decided to allow the use of the full dataset for reward estimation in the Q\#-HF algorithm. This modification aims to provide a more representative evaluation of its potential (albeit at the expense of more training data).

\textbf{Reward-Model Calibration:} Figure~\ref{fig:reward_hist} contrasts reward scores assigned by the BT model to correct versus incorrect generations produced by the baseline. A larger separation indicates stronger alignment between the reward and task success.

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{neurips2025/figures/histograms/figu-hist2.pdf}
    \caption{Distribution of learned reward scores w.r.t preferred/correct (green) and not preferred/incorrect (red) for ID(in-dist.)/OOD(out-of-dist.) data.  The reward function is difficult to learn.}
    \label{fig:reward_hist}
\end{figure}

==> arxiv/sections/app-d-experiments.tex <==
\section{EXPERIMENTS}\label{app:experiments}

\subsection{Math Reasoning}\label{app:math}

We benchmark \textbf{PITA} on the GSM8K grade-school arithmetic corpus~\cite{cobbe2021training}, which was also considered in the main paper.  However, in the main paper, PITA was evaluated with only a single round of training ($k=1$ in Algorithm 1). To achieve a fairer comparison, we extend the evaluation by running an additional round ($k=2$) of training to obtain a greater diversity of preference data. This iterative training process allows PITA to better adapt to the preferences, leading to more robust results in alignment tasks.

Additionally, in the main paper we evaluated the Q\#-HF algorithm with a reward function that was trained using only 50\% of the data to ensure that the total data used for both reward estimation and policy training was comparable to other algorithms. Given that Q\#-HF performed poorly in this setup, we decided to allow the use of the full dataset for reward estimation in the Q\#-HF algorithm. This modification aims to provide a more representative evaluation of its potential (albeit at the expense of more training data). 

\paragraph{Dataset.}  \textbf{GSM8K} contains \(7{,}500\) training and \(1{,}319\) test problems.  
We create a \(90\%/10\%\) split of the original training set for learning and validation, reserving the full test set for final reporting.

\paragraph{Models.}  We use the \textbf{Llama-3 8B-Instruct} model as our reference policy and the \textbf{Llama-3.2 1B-Instruct} model ~\cite{grattafiori2024llama} as the backbone for our Value function. For Q\#-HF, the reward model trained from preference data is also a Llama-3.2 1B-Instruct.

\paragraph{Algorithms.}  We evaluate the following approaches against the base reference model \(\pi_{\text{ref}}\):

\begin{itemize}[leftmargin=1.4em]
    \item \textbf{Q\#}:  The algorithm described in ~\cite{zhou2025q} trained directly on the GSM8K dataset with access to the true binary reward labels.  
    \item \textbf{Q\#-HF}:  A {\em two-stage} procedure: first, a reward model is trained from GSM8K preference pairs; this learned reward is then used in the Q\# algorithm to obtain the final policy.  
    \item \textbf{PITA (ours)}:  The algorithm described in Section~4, which learns a soft \(Q\)-function directly from preference data and induces the final policy without requiring a reward model from preference data.  
\end{itemize}

\paragraph{Training hardware.}   
All training and evaluation are performed on a single NVIDIA A100 80 GB GPU. 

\paragraph{Evaluation protocol.}  
We report single-sample accuracy (\textit{pass@1}) and majority-vote accuracy over \(k{=}\!8\) samples (\textit{maj1@8}).  
Generations use temperature \(T=0.8\) and nucleus sampling \(p=0.9\).

\begin{table}[H]
  \centering
  \caption{GSM8K accuracy (\%) and KL divergence.}
  \label{tab:pita-gsm8k-correct}
  \begingroup
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{lccc}
    \toprule
    \textbf{Algorithm} & \textbf{pass@1} & \textbf{maj1@8} & \textbf{KL}↓ \\
    \midrule
    $\pi_{\text{ref}}$  & 69.1 & 85.8 & - \\
    Q\#                 & 78.4 & 88.1 & 2.65 \\
    Q\#-HF              & 67.23 & 78.09 & 2.48 \\
    \midrule
    \textbf{PITA (ours)}& 75.92 & 86.81 & 21.67 \\
    \bottomrule
  \end{tabular}
  \endgroup
\end{table}

\textbf{Reward-Model Calibration in Q\#-HF:} Figure~\ref{fig:reward_hist_correct} contrasts reward scores assigned by the BT model to correct versus incorrect generations produced by the baseline. A larger separation indicates stronger alignment between the reward and task success. The reward model here was trained for 10 epochs, whereas the one in Figure~\ref{fig:reward_hist} was trained for half an epoch.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{neurips2025/figures/histograms/figu-hist-2.pdf}
    \caption{Distribution of learned reward scores w.r.t preferred/correct (green) and not preferred/incorrect (red) for ID(in-dist.)/OOD(out-of-dist.) data.  The reward function is better learned than earlier, given the greater data provided.}
    \label{fig:reward_hist_correct}
      %\vspace{-0.5in}
\end{figure}

\paragraph{Discussion.}  
Table~\ref{tab:pita-gsm8k-correct} shows that PITA attains performance on par with Q\# even without access to the true reward labels. Despite using a learned reward model with increased availability of preference data, Q\#-HF fails to perform as well as PITA, highlighting the brittleness of reward estimation in this setting. This suggests that PITA's preference-based approach is more robust and effective in aligning model outputs with desired preferences.

 Additionally, the KL-Divergence of PITA is higher than that of Q\# and Q\#-HF. This is because the language model used to provide preference feedback in PITA is OpenMathInstruct-2, which is distinct from the rule-based reward function score used in Q\#. This highlights the tradeoff between alignment with the reference policy and the flexibility of preference-based feedback.

% \subsection{Math Reasoning}\label{app:math}

% We benchmark \textbf{PITA} on the GSM8K grade-school arithmetic corpus~\cite{cobbe2021training}.

% \paragraph{Dataset.}  \textbf{GSM8K} contains \(7{,}500\) training and \(1{,}319\) test problems.  
% We create a \(90\%/10\%\) split of the original training set for learning and validation, reserving the full test set for final reporting.

% \paragraph{Models.}  We use the \textbf{Llama-3 8B-Instruct} model as our reference policy and the \textbf{Llama-3.2 1B-Instruct} model ~\cite{grattafiori2024llama} as the backbone for our Value function. For Q\#-HF the reward model trained from preference data is also a LLama-3.2 1B-Intstruct.


% \paragraph{Algorithms.}  We evaluate the following approaches against the base reference model \(\pi_{\text{ref}}\):

% \begin{itemize}[leftmargin=1.4em]
%     \item \textbf{Q\#}:  The algorithm described in ~\cite{zhou2025q} trained directly on GSM8K dataset with access to the true binary reward labels.  
%     \item \textbf{Q\#-HF}:  a {\em two-stage} procedure - first a reward model is trained from GSM8K preference pairs; this learned reward is then plugged into the Q\# algorithm to obtain the final policy.  
%     \item \textbf{PITA (ours)}:  the algorithm mentioned in of Section~4, which learns a soft \(Q\)-function directly from preference data and induces the final policy without having to learn a reward model from preference data.  
% \end{itemize}

% \paragraph{Training hardware.}   
% All training and evaluation are performed on a single NVIDIA A100 80 GB GPU. 

% \paragraph{Evaluation protocol.}  
% We report single-sample accuracy (\textit{pass@1}) and majority-vote accuracy over \(k{=}\!8\) samples (\textit{maj1@8}).  
% Generations use temperature \(T=0.8\) and nucleus sampling \(p=0.9\).

% \begin{table}[H]
%   \centering
%   \caption{GSM8K accuracy (\%) and KL divergence.}
%   \label{tab:pita-gsm8k-correct}
%   \begingroup
%   \setlength{\tabcolsep}{6pt}
%   \renewcommand{\arraystretch}{1.2}
%   \begin{tabular}{lccc}
%     \toprule
%     \textbf{Algorithm} & \textbf{pass@1} & \textbf{maj1@8} & \textbf{KL}↓ \\
%     \midrule
%     $\pi_{\text{ref}}$  & 69.1 & 85.8 & - \\
%     Q\#                 & 78.4 & 88.1 & 2.65 \\
%     Q\#-HF              & 67.23 & 78.09 & 2.48 \\
%     \midrule
%     \textbf{PITA (ours)}& 75.92 & 86.81 & 21.67 \\
%     \bottomrule
%   \end{tabular}
%   \endgroup
% \end{table}

% \textbf{Reward-Model Calibration in Q\#-HF:} Figure~\ref{fig:reward_hist_correct} contrasts reward scores assigned by the BT model to correct versus incorrect generations produced by the baseline. A larger separation indicates stronger alignment between the reward and task success. The reward model here was trained for 10 epochs, whereas the one in ~\ref{fig:reward_hist} was trained for half an epoch. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{neurips2025/figures/histograms/figu-hist-2.pdf}
%     \caption{Distribution of learned reward scores w.r.t preferred/correct (green) and not preferred/incorrect (red) for ID(in-dist.)/OOD(out-of-dist.) data.  The reward function is difficult to learn.}
%     \label{fig:reward_hist_correct}
% \end{figure}


% \paragraph{Discussions.}  
% Table~\ref{tab:pita-gsm8k-correct} shows that PITA attains performance on par with Q\# even without having knowledge of the true reward labels. Q\#-HF despite using a learnt reward model that is well aligned with the true reward signal as demonstrated in ~\ref{fig:reward_hist_correct} fails to perform as well as PITA.



%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Star-Graph Reasoning}

We demonstrate the effectiveness of \textbf{PITA} in guiding a reference language model (LM) to achieve near-perfect generalization accuracy on the star-graph task~\citep{bachmann2024pitfalls}, outperforming value-based baselines such as \textbf{Q\#}~\citep{zhou2025q} and \textbf{CD}~\citep{mudgal2023controlled}. A star-graph \(\mathcal{G}(d, l)\) is defined as a tree with \(d\) paths of length \(l\) emanating from a common root node. The task is for the LM to generate the correct path from the root to a leaf, given the edge set defining the graph. Figure~\ref{fig:star-graph} illustrates the star-graph task.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.9\textwidth]{neurips2025/figures/star-graph.pdf} % replace with your filename
  \caption{A \(\mathcal{G}= (3,8)\) star-graph configuration with degree \(d=3\), and path length \(l=8\). The pre-trained model, with next-token prediction, learns a faulty shortcut: it selects a random first node and follows the path from there on.}
  \label{fig:star-graph}
  %\vspace{-0.3in}
\end{figure}

Despite the task’s structural simplicity, \citet{bachmann2024pitfalls} highlight a key failure mode in models trained with next-token prediction. Specifically, the model often learns a \textit{Clever-Hans} shortcut—selecting the first node in the root’s adjacency list and following it to a leaf. While this heuristic yields perfect accuracy on the training set, it fails to generalize: on unseen test graphs, the model selects the correct path only with probability \(1/d\), since the first adjacent node is correct only \(1/d\) of the time.

\citet{zhou2025q} show that such faulty behavior can be corrected during post-training using value-based methods. However, widely used policy-based approaches like REINFORCE~\citep{ahmadian2024back}, DPO~\citep{rafailov2023direct}, and RPO~\citep{pang2024iterative} are unable to overcome this shortcut, achieving test accuracy no better than \(1/d\). This failure is likely due to the difficulty transformer-based architectures face when unlearning spurious heuristics via policy-gradient optimization~\citep{hu2024learning}.

We now describe the training methodology used to apply \textbf{PITA} to the star-graph task.

\textbf{Training Setup:} We follow the experimental setup of Q\#~\cite{zhou2025q} to generate and evaluate the star-graph datasets. We report test accuracies of PITA (ours) on three classes of graphs: smaller graphs \(\mathcal{G}(2, 5)\) and \(\mathcal{G}(5, 5)\), where we employ the GPT-2 small model, and a larger graph \(\mathcal{G}(3, 8)\), for which we use the GPT-2 medium model~\cite{radford2019language} to train the set of \textit{pre-trained models}. All models are initially pretrained using next-token prediction on a dataset of 200k randomly sampled graphs paired with their correct paths.

We consider several baselines, including \textbf{REINFORCE}, \textbf{DPO}, \textbf{RPO}—as well as value-based methods \textbf{Q\#} and \textbf{CD}. Post-training is conducted on a separate dataset of 200k new random graphs. To ensure a fair comparison, we reproduce the results with an identical reward structure and reuse the datasets used in~\cite{zhou2025q}. For REINFORCE, a reward of 1 is assigned for correct paths and \(-0.1\) for incorrect ones. For DPO and RPO, pairwise comparisons between a correct path \(y_{\text{chosen}}\) and an incorrect shortcut path \(y_{\text{reject}}\) are sampled from the pre-trained model. Similarly, for \textbf{Q\#}, a classifier is trained on the same pairwise dataset, labeling correct paths with reward 1 and incorrect ones with 0. Note that PITA uses a unique reference generation at the core of its algorithm. In PITA, we treat correct paths as the \textit{`preferred'} solution and the incorrect path as the \textit{`not-preferred'} answer to estimate the preference distribution. The unique correct answer naturally serves as the reference completion for the star-graph task. We report our test results in Table~\ref{tab:pita-star-graph}.

\begin{table}[h]
    \centering
    \caption{Comparison of PITA with other baselines across star-graph configurations.}
    \label{tab:pita-star-graph}
    \begingroup
    \setlength{\tabcolsep}{6pt}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Algorithm} & $\mathcal{G}(2,5)$ & $\mathcal{G}(5,5)$ & $\mathcal{G}(3,8)$ \\
        \midrule
        pre-trained & 49.94 & 19.8 & 33.24 \\
        Q\# & 99.90 & 97 & 98.62 \\
        CD & 99.94 & 98.62 & 99.52 \\
        REINFORCE & 49.19 & 13.13 & 25.96 \\
        DPO & 37.61 & 0.0 & 0.0 \\
        RPO & 49.69 & 19.93 & 33.47 \\
        \midrule
        \textbf{PITA (ours)} & 99.97 & 99.7 & 99.93 \\
        \bottomrule
    \end{tabular}
    \endgroup
\end{table}

All models are trained for 10 epochs using the AdamW optimizer with a weight decay of $0.1$ and a batch size of $256$. The learning rates are set to $2.5 \times 10^{-4}$ for pretraining, $1 \times 10^{-5}$ for REINFORCE, and $1 \times 10^{-4}$ for DPO, RPO, CD, and Q\#. For Q\# and CD, we set the inverse temperature parameter $\eta = 0.1$. Training is performed on a single A100 GPU. Evaluation is conducted on a held-out test set of 20k graphs using top-$k = 10$ sampling and temperature $1.0$.

\paragraph{Discussion.}  
The star-graph experiments provide valuable insights into why PITA outperforms standard policy-based methods, as well as other value-based algorithms like Q\# and CD. While REINFORCE achieves a maximum accuracy of \(1/d\), the performance of DPO is significantly worse. We observe similar behavior to that reported in~\cite{zhou2025q}, where DPO achieves \(0\) accuracy, with the policy collapsing probabilities to \(0\). In contrast, value-based methods perform better across all graph configurations. Notably, PITA achieves further performance improvements, even when baseline reward-based methods are already near perfect accuracy. This improvement in accuracy can be attributed to PITA's ability to generate more precise implicit rewards. Upon examining the rewards generated by Q\# for the star-graph reasoning test set, we find that the reward differences between correct and incorrect answers are significantly smaller compared to those generated by PITA.


% The star-graph experiments provide insight into why PITA is effective compared to standard policy-based methods, and even other value-based algorithms like Q\# and CD. While REINFORCE has an accuracy of at most \(1/d\), the performance of DPO is lacking. We observe similar behavior as reported in~\cite{zhou2025q} with \(0\) accuracy for DPO, where the policy collapses the probabilities to \(0\). In contrast, the value-based methods achieve better performance across all graph configurations. In particular, we would like to highlight the performance gains of PITA, even though it is already close to perfect accuracy with baselines based on reward-based methods. The increase in accuracy is due to finer implicit reward generation by PITA. Taking a closer look at the rewards generated by Q\# for the star-graph reasoning task test set, we observe that the difference in rewards assigned between correct and incorrect answers is significantly lower compared to what PITA generates.




% In this section, we demonstrate the effectiveness of \textbf{PITA} in guiding a reference language model (LM) to achieve near-perfect generalization accuracy on the star-graph task~\cite{bachmann2024pitfalls}, outperforming value-based baselines such as \textbf{Q\#}~\cite{zhou2025q} and \textbf{CD}~\cite{mudgal2023controlled}. A star-graph $\mathcal{G}(d, l)$ is defined as a tree with $d$ paths of length $l$ emanating from a common root node. The goal is for the LM to generate the correct path from the root to a leaf, given the edge set defining the graph. Figure~\ref{fig:star-graph} illustrates the star-graph task.

% \begin{figure}[H]
%   \centering
%   \includegraphics[width=\textwidth]{neurips2025/figures/star-graph.pdf} % replace with your filename
%   \caption{A $\cG= (3,8)$ star-graph configuration with degree $d=3$, and path length $l=8$. Pre-trained model with next-token prediction, learns a faulty shortcut which selects a random first node, and follow the path from there on.}
%   \label{fig:star-graph}
%   \vspace{-0.2in}
% \end{figure}

% Despite the task’s structural simplicity, \cite{bachmann2024pitfalls} highlight a key failure mode in models trained with next-token prediction. Specifically, the model often learns a \textit{Clever-Hans} shortcut—selecting the first node in the root’s adjacency list and following it to a leaf. While this heuristic yields perfect accuracy on the training set, it fails to generalize: on unseen test graphs, the model selects the correct path only with probability $1/d$, since the first adjacent node is correct only $1/d$ of the time.

% Zhou et al.~\cite{zhou2025q} show that such faulty behavior can be corrected during post-training using value-based methods. However, widely used policy-based approaches like REINFORCE~\cite{ahmadian2024back}, DPO~\cite{rafailov2023direct}, and RPO~\cite{pang2024iterative} are unable to overcome this shortcut, achieving test accuracy no better than $1/d$. This failure is likely due to the difficulty transformer-based architectures face when unlearning spurious heuristics via policy-gradient optimization~\cite{hu2024learning}.

% We now describe the training methodology used to apply \textbf{PITA} to the star-graph task.

% \textbf{Training Setup:} We closely follow the experimental setup of Q\#~\cite{zhou2025q} to generate and evaluate the star-graph datasets. We report test accuracies of PITA(ours) on three classes of graphs smaller graphs $\mathcal{G}(2, 5)$ and $\mathcal{G}(5, 5)$, where we employ the GPT-2 small model, and a larger graph $\mathcal{G}(3, 8)$, for which we use the GPT-2 medium model~\cite{radford2019language} to train the set of \textit{pre-trained models}.
% All models are initially pretrained using next-token prediction on a dataset of 200k randomly sampled graphs paired with their correct paths. 

% We consider several baselines which include \textbf{REINFORCE},\textbf{DPO},\textbf{RPO}—as well as value-based methods \textbf{Q\#} and \textbf{CD}. Post-training is conducted on a separate dataset of 200k new random graphs.
% In order to have a fair comparison, we reproduce the results with identical reward structure, and reuse the datasets used in~\cite{zhou2025q}.
% For REINFORCE, a reward of $1$ is assigned for correct paths and $-0.1$ for incorrect ones.
% For DPO and RPO, pairwise comparisons between a correct path $y_{\text{chosen}}$ and an incorrect shortcut path $y_{\text{reject}}$ are sampled from the pre-trained model. Similarly, for \textbf{Q\#}, a classifier is trained on the same pairwise dataset, labeling correct paths with reward $1$ and incorrect ones with $0$. Note that PITA uses a unique reference generation at the core of it's algorithm.
% In PITA, we treat correct paths as the \textit{`preferred'} solution and the incorrect path as the \textit{`not-preferred'} answer to estimate the preference distribution. The unique correct answer naturally serves as the reference completion for the star-graph task.
% We report our test results in Table~\ref{tab:pita-star-graph}

% \begin{table}[H]
%     \centering
%     \caption{Comparison of PITA with other baselines across star-graph configurations.}
%     \label{tab:pita-star-graph}
%     \begingroup
%     \setlength{\tabcolsep}{6pt}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lccc}
%         \toprule
%         \textbf{Algorithm} & $\mathcal{G}(2,5)$ & $\mathcal{G}(5,5)$ & $\mathcal{G}(3,8)$ \\
%         \midrule
%         pre-trained & 49.94 & 19.8 & 33.24 \\
%         Q\# & 99.90 & 97 & 98.62 \\
%         CD & 99.94 & 98.62 & 99.52 \\
%         REINFORCE & 49.19 & 13.13 & 25.96 \\
%         DPO & 37.61 & 0.0 & 0.0 \\
%         RPO & 49.69 & 19.93 & 33.47 \\
%         \midrule
%         \textbf{PITA (ours)} & 99.97 & 99.7 & 99.93 \\
%         \bottomrule
%     \end{tabular}
%     \endgroup
% \end{table}


% All models are trained for 10 epochs using the AdamW optimizer with a weight decay of $0.1$ and a batch size of $256$. The learning rates are set to $2.5 \times 10^{-4}$ for pretraining, $1 \times 10^{-5}$ for REINFORCE, and $1 \times 10^{-4}$ for DPO, RPO, CD, and Q\#. For Q\# and CD, we set the inverse temperature parameter $\eta = 0.1$. Training is performed on a single A100 GPU. Evaluation is conducted on a held-out test set of 20k graphs using top-$k = 10$ sampling and temperature $1.0$.

% \textbf{Discussion.}
% The star-graph experiments provides us insight into why PITA is effective compared to the standard policy based methods, and even the other value based algorithms like $Q\#$ and CD. While REINFORCE has an accuracy of at most $1/d$, the performance of DPO is lacking. We observe a similar behavior as reported in~\cite{zhou2025q} with $0$ accuracy for DPO where the policy collapses the probabilities to 0. In contrast the value based methods achieve better performance across all graph configurations. In particular, we would like to highlight the performance gains of PITA despite already close to perfect accuracy with baselines based on reward based methods. We notice that the increase in accuracy is due to finer implicit reward generation by PITA. Taking a closer look at the rewards generated by $Q\#$ for the star graph reasoning task test set, the difference of rewards assigned between correct and incorrect answers are significantly lower compared to what PITA gives.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{IMDB Sentiment Generation}\label{app:imdb}

We next evaluate \textbf{PITA} on controlled sentiment generation. The task follows the IMDB-Gen setting of ~\cite{ramamurthy2023reinforcementlearningnotnatural} and ~\cite{chaudhary2025riskaversefinetuninglargelanguage}. Given the first 60 tokens of a movie review, the language model must continue the text so that the completed review expresses maximally positive sentiment.

\paragraph{Dataset.} We use the \textbf{IMDB Reviews} dataset, which contains \(25{,}000\) training and \(25{,}000\) test reviews, each labeled \emph{positive} or \emph{negative}. For each example, we truncate the review to its first 60 tokens, which form the prompt \(x\); the model then generates up to 60 continuation tokens \(y\). The reward model for this task is the \textbf{lvwerra/distilbert-imdb} classifier, with the logit corresponding to the positive sentiment output node used as the scalar reward. For the creation of the preference dataset, we select the generation with the higher reward as the preferred generation.

\paragraph{Models.} For this task, we use \textbf{TinyLlama-1.1B-Chat}\footnote{\url{https://huggingface.co/TinyLlama/TinyLlama-1.1B-Chat}} as both our reference policy and the backbone for our value function. For the reward model learned from the preference data for Q\#-HF, we use a \textbf{LLama 3.2 1B-Instruct} model.

\paragraph{Evaluation} We evaluate the same set of algorithms as above. For each of the \(5{,}000\) \textbf{IMDB} test set prompts, we sample a \emph{single} continuation using nucleus sampling with top-\(p = 0.9\) and temperature \(T = 0.8\). The full prompt + completion is scored by the \texttt{lvwerra/distilbert-imdb} sentiment classifier. We report the mean sentiment logit score (\textsc{Sent.}↑) and the token-level KL divergence (\textsc{KL}↓) between the fine-tuned policy and the reference model \(\pi_{\text{ref}}\).  An example of the completions generated by $\pi_{\text{ref}}$ and by PITA is shown in Figure~\ref{fig:imdb_example}.

\begin{table}[H]
  \centering
  \caption{IMDB-Gen: sentiment (higher is better) and KL divergence (lower is better) on 5,000 test prompts.}
  \label{tab:pita-imdb}
  \begingroup
  \setlength{\tabcolsep}{8pt}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{lcc}
    \toprule
    \textbf{Algorithm} & \textsc{Sent.}↑ & \textsc{KL}↓ \\
    \midrule
    $\pi_{\text{ref}}$ & -0.52 & - \\
    Q\#                & 0.22 & 7.51 \\
    Q\#-HF             & -0.44 & 5.22 \\
    \midrule
    \textbf{PITA (ours)} & 0.01 & 7.27 \\
    \bottomrule
  \end{tabular}
  \endgroup
\end{table}

\paragraph{Discussion.} The range of rewards generated by \texttt{lvwerra/distilbert-imdb} typically lies between -3 and +3. Q\# with access to true rewards performs the best. Among the algorithms that only have access to a preference signal, rather than the true reward, PITA performs the best. 

Sentiment alignment is inherently difficult, and Q\# has access to a pre-trained DistilBERT model specifically tuned for sentiment analysis. In contrast, reproducing a preference function with a similar structure requires much more preference data. Despite this challenge, PITA is able to extract valuable information from the given preference data and significantly outperforms Q\#-HF, which appears to have poorly learned a reward model. This demonstrates PITA's ability to leverage limited preference data for effective alignment.



%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%

% \subsection{IMDB Sentiment Generation}\label{app:imdb}

% We next evaluate \textbf{PITA} on controlled sentiment generation.  The task follows the IMDB-Gen setting of ~\cite{ramamurthy2023reinforcementlearningnotnatural} and ~\cite{chaudhary2025riskaversefinetuninglargelanguage}. Given the first 60 tokens of a movie review, the language model must continue the text so that the completed review expresses maximally positive sentiment.

% \paragraph{Dataset.}
% We use the \textbf{IMDB Reviews} dataset that contains \(25{,}000\) training and \(25{,}000\) test reviews, each labelled \emph{positive} or \emph{negative}.  
% For every example we truncate the review to its first 60 tokens, which form the prompt \(x\); the model then generates up to 60 continuation tokens \(y\).  The reward model for this task is the \textbf{lvwerra/distilbert-imdb} classifier. We use the logit corresponding to the positive sentiment output node as the scalar reward. For the creation of a preference dataset we simply choose the generation with a higher reward as the preferred generation.  

% \paragraph{Models.}
% For this task we use \textbf{TinyLlama-1.1B-Chat} \footnote{\url{https://huggingface.co/TinyLlama/TinyLlama-1.1B-Chat}} as both our reference policy and the backbone for our value function.  
% For the reward model learnt from the preference data for Q\#-HF we use a \textbf{LLama 3.2 1B-Instruct} model.



% \paragraph{Evaluation}
% We evaluate the same set of algorithms as above. For each of the \(5{,}000\) \textbf{IMDB} test set prompts we sample a \emph{single} continuation using nucleus sampling with top-\(p = 0.9\) and temperature \(T = 0.8\).  
% The full prompt + completion is scored by the \texttt{lvwerra/distilbert-imdb} sentiment classifier.  
% We report the mean sentiment logit score (\textsc{Sent.}↑) and the token-level KL divergence (\textsc{KL}↓) between the fine-tuned policy and the reference model \(\pi_{\text{ref}}\).

% \begin{table}[H]
%   \centering
%   \caption{IMDB-Gen: sentiment (higher is better) and KL divergence (lower is better) on 5 000 test prompts.}
%   \label{tab:pita-imdb}
%   \begingroup
%   \setlength{\tabcolsep}{8pt}
%   \renewcommand{\arraystretch}{1.2}
%   \begin{tabular}{lcc}
%     \toprule
%     \textbf{Algorithm} & \textsc{Sent.}↑ & \textsc{KL}↓ \\
%     \midrule
%     $\pi_{\text{ref}}$ & -0.52 & - \\
%     Q\#                & 0.22 & 7.51 \\
%     Q\#-HF             & -0.44 & 5.22 \\
%     \midrule
%     \textbf{PITA (ours)} & 0.01 & 7.27 \\
%     \bottomrule
%   \end{tabular}
%   \endgroup
% \end{table}

% \paragraph{Discussion.} The range of rewards generated by \texttt{lvwerra/distilbert-imdb} typically lies between -3 to +3. Q\# with access to true rewards performs the best. Among the algorithms that only have access to a preference signal as opposed to the true reward PITA performs the best. 

% We attribute the inability of PITA to perform as well as Q\# in this task to the lack of preference data compared to math reasoning task. (Here we have 5 )

\begin{figure}[ht]
\centering
\begin{minipage}{\textwidth}
\begin{tcolorbox}[colback=white, colframe=black]

\textbf{Prompt:} Paul Mazursky misfires on this film. The writing, direction, casting, and acting (with the exception of Victorio Gassman) are all off the mark. I remember the reviews from 20+ years ago being mediocre, but I thought it still might

\dasheddline

\textbf{Completion from $\pi^{\text{ref}}$:} \textcolor{red!80!black}{be good. But by today's standards, the film just isn't good enough. It's a muddled and overly long (about 2 1/2 hours) film that ultimately does not live up to its potential as a classic film noir.
}\\ 
\dasheddline

\textbf{Completion from PITA:} \textcolor{blue!30!green}{be good. I'm glad to see how far it's come. This is not a great film, but it's definitely a lot better than the original. I think that makes it more enjoyable to watch. The acting is excellent, with a lot of great performances by both Mar
}





\end{tcolorbox}
\end{minipage}
\caption{Comparison of IMDB review completions (constrained to 60 tokens) from $\pi_{\text{ref}}$ vs PITA.  PITA is able to change the sentiment positive, while $\pi_{\text{ref}}$ fails to do so.}  % involving book fractions.}
\label{fig:imdb_example}
\end{figure}




==> arxiv/sections/checklist.tex <==
\nextpage
\setcounter{page}{1}
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
  \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction accurately summarize the core contributions of the paper, specifically the introduction of the PITA framework for preference-guided inference-time alignment. This is consistent with the subsequent experimental results and theoretical analysis.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide a discussion of limitations in multiple sections: key assumptions are addressed
in Section 5, limitations are outlined in the conclusion, and additional details are available in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
      \item[] Answer: \answerYes{}
    \item[] Justification: Theoretical assumptions are clearly stated in the form of Assumptions \ref{assum:theta_bound} and \ref{assum:emb-norm-bound}, and the proofs for the results, such as Lemma \ref{eqn:mle} and the regret bounds, are provided with detailed justifications in the main paper and the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
   \item[] Answer: \answerYes{}
    \item[] Justification: The paper provides details about the experimental setup, including datasets, models, and evaluation metrics. The code and data are provided in the supplement.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
     \item[] Answer: \answerYes{}
    \item[] Justification: The code and data are provided in the supplement.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
       \item[] Answer: \answerYes{}
    \item[] Justification: The paper specifies the datasets used (e.g., GSM8Ketc.), the experimental setup, and evaluation tasks. 
 Details on parameter choices are available in the supplemental material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: We report statistical significance tests for the experimental results as appropriate.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: We specify the compute resources required for the experiments and type of hardware used.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
     \item[] Answer: \answerYes{}
    \item[] Justification: The paper adheres to the NeurIPS Code of Ethics, with no issues concerning ethics violations. The work focuses on aligning LLMs with user preferences, avoiding harmful or unintended consequences.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
     \item[] Answer: \answerYes{}
    \item[] Justification: The paper discusses the potential positive impact of more efficient and controlled LLMs, while acknowledging the challenges of data quality and the risk of generating biased outputs in certain applications.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper uses publicly available datasets and models, and the alignment approaches do not result in any new models with high misuse potential.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification:  All original owners of assets (e.g., code, data, models) are properly cited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: The introduced assets are documented and will be released along with the code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
     \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve any crowdsourcing or human subject research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve human subjects, so IRB approval is not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
   \item[] Answer: \answerYes{}
    \item[] Justification: The paper clearly describes the use of LLMs in the context of preference-guided inference-time alignment and discusses how these models are integrated into the proposed method.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> arxiv/sections/experiments-v2.tex <==
\section{Experimental Evaluation}\label{sec:experiments}

We adopt the experimental setup from Q\#, as it serves as one of the benchmarks against which we compare the performance of PITA. To ensure consistency, we use the same base models and datasets. In this section, we provide an overview of the experimental setup, while additional details on datasets, training, and evaluation criteria are provided in Appendix~\ref{app:experiments}. All experiments were run on machines equipped with a single NVIDIA A100 80 GB GPU. Our code is available at \url{https://anonymous.4open.science/r/pref-sharp-D223}.

We empirically evaluate the proposed \textbf{PITA} algorithm on mathematical reasoning tasks and compare it against a strong reward-model baseline. Our study focuses on three key questions: 1) Does PITA improve task accuracy (\textit{pass@1} and \textit{maj@8}) over a baseline using post-training Q\# with a learned preference reward model? 2) Does the KL divergence to the reference policy remain controlled? 3) How well does the learned reward model discriminate between correct and incorrect generations?

\subsection{Experimental Setup}\label{subsec:setup}

\textbf{Datasets.} We evaluate our algorithm on the arithmetic reasoning dataset GSM8K~\cite{cobbe2021training}. GSM8K (Grade School Math 8K) is a dataset containing 8.5K high-quality, linguistically diverse math word problems aimed at the grade school level. These problems, designed for question-answering tasks, require 2 to 8 steps and involve basic arithmetic operations. For test set evaluation, we use the entire GSM8K test set to evaluate the performance of the trained PITA model~\cite{lightman2023let,wang2023math}.

\textbf{Models.} We use the Llama 3~\cite{grattafiori2024llama} family of models to train our preference function, as they are highly competitive in arithmetic reasoning tasks~\cite{zhou2025q}.

\textbf{Metrics.} We report \emph{pass@1} (exact-match accuracy of the highest-ranking sample), \emph{maj@8} (majority-vote accuracy over 8 samples), and the forward KL divergence $\text{KL}(\pi\,\Vert\,\pi_{\text{ref}})$ computed on the \textsc{GSM8K} test set. Lower KL values indicate closer adherence to the reference policy.

\textbf{Algorithms.} We compare the performance of the following algorithms on the GSM8K dataset against the base reference model $\pi_{\mathrm{ref}}$:\\
\textbf{Q\#}: The trained Q\# model is evaluated for its accuracy on the GSM8K dataset.\\
\textbf{Q\#-HF}: We first train a reward model using preference data derived from the GSM8K dataset, then use this reward model in the Q\# algorithm to train the final model.\\
\textbf{PITA (ours)}: The iterative approach described in Section~\ref{sec:PITA} is used to learn an optimal soft-Q function from preference data derived from the GSM8K dataset. The final model, induced by the learned $Q$-function, is then evaluated.

\textbf{Training details.} Each optimization run uses a single NVIDIA A100 GPU. PITA trains for 10 policy-evaluation/optimization cycles, each with a learning rate of $2 \times 10^{-5}$ and a context length of 4096. The baseline uses identical hyperparameters.

\textbf{Comparison of Algorithms:} In Table~\ref{tab:gsm8k_main}, we compare the performance of the above algorithms. The reference model $\pi_{\mathrm{ref}}$ is chosen to be the Llama 3 8B model. We observe that PITA significantly outperforms Llama3 on both \textbf{pass@1} accuracy and \textbf{maj@8} evaluation metrics. Additionally, the performance gap between PITA and Q\# appears to be small.

\begin{table}[h]
    \centering
    \caption{Performance on the \textsc{GSM8K} \emph{test} split.}
    \label{tab:gsm8k_main}
    \begingroup
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Algorithm} & \textbf{pass@1} $\uparrow$ & \textbf{maj@8} $\uparrow$ & \textbf{KL}  \\
        \midrule
        $\pi_{\mathrm{ref}}$ & 69 & 85 & - \\
        Q\# & 78.4 & 88.1 & 2.65 \\
        Q\#-HF & 49.9 & 72.0 & 18.85 \\
        \midrule
        PITA (ours)  & 74.8 & 86.1 & 18.4 \\
        \bottomrule
    \end{tabular}
    \endgroup
\end{table}
\textbf{Reward-Model Calibration:} Figure~\ref{fig:reward_hist} contrasts reward scores assigned by the BT model to correct versus incorrect generations produced by the baseline. A larger separation indicates stronger alignment between the reward and task success.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{neurips2025/figures/histograms/figu-hist2.pdf}
    \caption{Distribution of learned reward scores w.r.t preferred/correct (green) and not preferred/incorrect (red) for ID(in-dist.)/OOD(out-of-dist.) data.  The reward function is difficult to learn.}
    \label{fig:reward_hist}
\end{figure}

\textbf{Discussion:} We observe that PITA significantly outperforms the Q\#-HF baseline on both accuracy metrics while maintaining comparable or lower KL divergence. The poor performance of Q\#-HF can be attributed to the brittleness of its reward estimation process, which has failed to provide stable guidance during training. This demonstrates that iterative policy optimization with sparse rewards, as used in PITA, is more sample-efficient than single-stage MLE fine-tuning. PITA’s approach not only improves task performance but also reduces the need for large amounts of labeled preference data, making it more computationally efficient. Furthermore, PITA's ability to maintain alignment with the reference policy while improving accuracy highlights its robustness in real-world applications. Additional insights and tasks are presented in Appendix~\ref{app:experiments}.

%We observe that PITA outperforms the Q\#-HF baseline on both accuracy metrics while maintaining comparable or lower KL divergence, demonstrating that iterative policy optimization with sparse rewards is more sample-efficient than single-stage MLE fine-tuning. This suggests that PITA's approach to preference-guided learning is not only effective but also more computationally efficient, reducing the need for large amounts of labeled preference data. Furthermore, PITA's ability to maintain alignment with the reference policy while improving task performance highlights its robustness in real-world applications. Additional tasks are presented in Appendix~\ref{app:experiments}.

%We observe that PITA outperforms the Q\#-HF baseline on both accuracy metrics while maintaining comparable or lower KL divergence, demonstrating that iterative policy optimization with sparse rewards is more sample-efficient than single-stage MLE fine-tuning. Additional tasks are presented in Appendix~\ref{app:experiments}.

==> arxiv/sections/experiments-v3.tex <==
\section{Experimental Evaluation}\label{sec:experiments}

We adopt the experimental setup from Q\#, as it serves as one of the benchmarks against which we compare the performance of PITA. To ensure consistency, we use the same base models and datasets. In this section, we provide an overview of the experimental results, while additional details on datasets, training, and evaluation criteria are provided in Appendix~\ref{app:experiments}. All experiments were run on machines equipped with a single NVIDIA A100 80 GB GPU. Our code is available at \url{https://anonymous.4open.science/r/pref-sharp-D223}.



\subsection{Experimental Setup}\label{subsec:setup}

\textbf{Models and Datasets.} 
We perform PITA training using the following models: Meta-Llama-3-8B-Instruct, Meta-Llama-3.2-1B-Instruct, TinyLlama-1.1B-Chat-v1.0, GPT-2 small, medium models.
We evaluate our algorithm on three diverse tasks with varying difficulty levels: arithmetic reasoning GSM8K~\cite{cobbe2021training}, star-graph reasoning~\cite{bachmann2024pitfalls}, and sentiment generation~\cite{chaudhary2025riskaversefinetuninglargelanguage}.
We use the Llama 3~\cite{grattafiori2024llama} family of models to train our preference function, as they are highly competitive in arithmetic reasoning tasks~\cite{zhou2025q}. The GPT-2 small, and medium models are used for training in star graph reasoning similar to the framework in ~\cite{bachmann2024pitfalls}.  For sentiment generation, we use the TinyLlama 1.1 B model following~\cite{chaudhary2025riskaversefinetuninglargelanguage}. 






\textbf{Metrics.} We report \emph{pass@1} (exact-match accuracy of the highest-ranking sample), \emph{maj@8} (majority-vote accuracy over 8 samples), and the forward KL divergence $\text{KL}(\pi\,\Vert\,\pi_{\text{ref}})$ computed on the \textsc{GSM8K} test set. Lower KL values indicate closer adherence to the reference policy.







\subsection{Algorithms}
% We compare the performance of the following algorithms on the GSM8K dataset against the base reference model $\pi_{\mathrm{ref}}$:\\

% \begin{itemize}[leftmargin=1.4em]
%     \item \textbf{Q\#}:  The algorithm described in ~\cite{zhou2025q} trained directly on the GSM8K dataset with access to the true binary reward labels.  
%     \item \textbf{Q\#-HF}:  A {\em two-stage} procedure: first, a reward model is trained from GSM8K preference pairs; this learned reward is then used in the Q\# algorithm to obtain the final policy.  
%     \item \textbf{PITA (ours)}:  The algorithm described in Section~4, which learns a soft \(Q\)-function directly from preference data and induces the final policy without requiring a reward model from preference data.  
% \end{itemize}

% For star graph reasoning, we also compare the performance of PITA with the following algorithms.
% \begin{itemize}[leftmargin=1.4em]
%     \item \textbf{CD}:  The algorithm described in ~\cite{zhou2025q} trained directly on the GSM8K dataset with access to the true binary reward labels.  
%     \item \textbf{REINFORCE}:  A {\em two-stage} procedure: first, a reward model is trained from GSM8K preference pairs; this learned reward is then used in the Q\# algorithm to obtain the final policy.  
%     \item \textbf{DPO}:  The algorithm described in Section~4, which learns a soft \(Q\)-function directly from preference data and induces the final policy without requiring a reward model from preference data.
%     \item \textbf{RPO}:  The algorithm described in Section~4, which learns a soft \(Q\)-function directly from preference data and induces the final policy without requiring a reward model from preference data.
% \end{itemize}


We compare the performance of the following algorithms against the base reference model $\pi_{\mathrm{ref}}$:

\begin{itemize}[leftmargin=1.4em]
    \item \textbf{Q\#}: The algorithm described in~\cite{zhou2025q}, trained directly using access to true binary reward labels.  
    \item \textbf{Q\#-HF}: A {\em two-stage} procedure: first, a reward model is trained from preference pairs (so called ``human feedback''); this learned reward is then used in the Q\# algorithm to obtain the final policy.  
    \item \textbf{PITA (ours)}: The algorithm described in Section~4, which learns a soft \(Q\)-function directly from preference data and induces the final policy without requiring a separate reward model.
\end{itemize}

For star graph reasoning, we also compare the performance of PITA with the following algorithms:

\begin{itemize}[leftmargin=1.4em]
    \item \textbf{CD}: The algorithm described in~\cite{mudgal2023controlled}, trained directly using access to true binary reward labels.  
    \item \textbf{REINFORCE}: A post-training algorithm that uses REINFORCE instead of the canonical Proximal Policy Optimization (PPO) for the RL part of Reinforcement Learning from Human Feedback.  
    \item \textbf{DPO}: A post-training algorithm that directly aligns language models using human preferences by optimizing for preferred responses over less preferred ones without requiring reinforcement learning.
    \item \textbf{RPO}: A post-training algorithm that uses a modified DPO loss to improve accuracy on reasoning tasks.
\end{itemize}



% \begin{description}
%   \item[\textbf{Q\#}]
%   The trained Q\# model is evaluated for its accuracy on the GSM8K dataset.
%   \item[\textbf{Q\#-HF}]
%   We first train a reward model using preference data derived from the GSM8K dataset, then use this reward model in the Q\# algorithm to train the final model.
%   \item[\textbf{PITA (ours)}]
%   The iterative approach described in Section~\ref{sec:PITA} is used to learn an optimal soft-Q function from preference data derived from the GSM8K dataset. The final model, induced by the learned $Q$-function, is then evaluated.
% \end{description}


\subsection{Main Results}\label{subsec:main-results}
We present our main results for the performance of our algorithm on the arithmetic reasoning dataset GSM8K~\cite{cobbe2021training}. GSM8K (Grade School Math 8K) is a dataset containing 8.5K high-quality, linguistically diverse math word problems aimed at the grade school level. These problems, designed for question-answering tasks, require 2 to 8 steps and involve basic arithmetic operations. For test set evaluation, we use the entire GSM8K test set to evaluate the performance of the trained PITA model~\cite{lightman2023let,wang2023math}.

In Table~\ref{tab:gsm8k_main}, we compare the performance PITA and other value-guided algorithms to the reference model $\pi_{\mathrm{ref}}$. The reference model $\pi_{\mathrm{ref}}$ is chosen to be the Llama 3 8B model. We observe that PITA significantly outperforms Llama3 on both \textbf{pass@1} accuracy and \textbf{maj@8} evaluation metrics. Additionally, the performance gap between PITA and Q\# appears to be small. Training details for PITA are given in Appendix~\ref{app:experiments}

\begin{table}[H]
  \centering
  \caption{GSM8K accuracy (\%) and KL divergence.}
  \label{tab:gsm8k_main}
  \begingroup
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{lccc}
    \toprule
    \textbf{Algorithm} & \textbf{pass@1} & \textbf{maj1@8} & \textbf{KL}↓ \\
    \midrule
    $\pi_{\text{ref}}$  & 69.1 & 85.8 & - \\
    Q\#                 & 78.4 & 88.1 & 2.65 \\
    Q\#-HF              & 67.23 & 78.09 & 2.48 \\
    \midrule
    \textbf{PITA (ours)}& 75.92 & 86.81 & 21.67 \\
    \bottomrule
  \end{tabular}
  \endgroup
\end{table}

\textbf{Reward-Model Calibration in Q\#-HF:} Figure~\ref{fig:reward_hist_correct} contrasts reward scores assigned by the BT model to correct versus incorrect generations produced by the baseline. A larger separation indicates stronger alignment between the reward and task success. The performance of Q\#-HF is highly sensitive to the reward training process as we see in an ablation study of reward training from preference data presented in Appendix~\ref{app:additonal-experiments}.


\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{neurips2025/figures/histograms/figu-hist-2.pdf}
    \caption{Distribution of learned reward scores w.r.t preferred/correct (green) and not preferred/incorrect (red) for ID(in-dist.)/OOD(out-of-dist.) data.  The reward function is better learned than earlier, given the greater data provided~\ref{app:additonal-experiments}}
    \label{fig:reward_hist_correct}
      %\vspace{-0.5in}
\end{figure}

Table~\ref{tab:gsm8k_main} shows that PITA attains performance on par with Q\# even without access to the true reward labels. Despite using a learned reward model with increased availability of preference data, Q\#-HF fails to perform as well as PITA, highlighting the brittleness of reward estimation in this setting. This suggests that PITA's preference-based approach is more robust and effective in aligning model outputs with desired preferences.

 Additionally, the KL-Divergence of PITA is higher than that of Q\# and Q\#-HF. This is because the language model used to provide preference feedback in PITA is OpenMathInstruct-2~\cite{toshniwal2024openmathinstruct}, which is distinct from the rule-based reward function score used in Q\#. This highlights the tradeoff between alignment with the reference policy and the flexibility of preference-based feedback.



\subsection{Effectiveness of PITA and Value-guided algorithms}
To better understand the effectiveness of our method in guiding a reference model at test time, we analyze the behavior of \textsc{PITA} alongside other value-guided algorithms, such as   \textbf{Q\#}~\citep{zhou2025q} and  \textbf{CD}~\citep{mudgal2023controlled}, on star-graph reasoning tasks~\citep{bachmann2024pitfalls}.
We observe that \textbf{PITA} effectively guides the reference language model (LM) to achieve near-perfect generalization accuracy on the star-graph task, outperforming strong value-based baselines such as \textsc{Q\#} and \textsc{CD}, which themselves exhibit high generalization performance.


\subsubsection{Star-Graph Reasoning}

 A star-graph \(\mathcal{G}(d, l)\) is defined as a tree with \(d\) paths of length \(l\) emanating from a common root node. The task is for the LM to generate the correct path from the root to a leaf, given the edge set defining the graph. Figure~\ref{fig:star-graph} illustrates the star-graph task.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.9\textwidth]{neurips2025/figures/star-graph.pdf} % replace with your filename
  \caption{A \(\mathcal{G}= (3,8)\) star-graph configuration with degree \(d=3\), and path length \(l=8\). The pre-trained model, with next-token prediction, learns a faulty shortcut: it selects a random first node and follows the path from there on.}
  \label{fig:star-graph}
  %\vspace{-0.3in}
\end{figure}

Despite the task’s structural simplicity, \citet{bachmann2024pitfalls} highlight a key failure mode in models trained with next-token prediction. Specifically, the model often learns a \textit{Clever-Hans} shortcut—selecting the first node in the root’s adjacency list and following it to a leaf. While this heuristic yields perfect accuracy on the training set, it fails to generalize: on unseen test graphs, the model selects the correct path only with probability \(1/d\), since the first adjacent node is correct only \(1/d\) of the time.

\citet{zhou2025q} show that such faulty behavior can be corrected during post-training using value-based methods. However, widely used policy-based approaches like REINFORCE~\citep{ahmadian2024back}, DPO~\citep{rafailov2023direct}, and RPO~\citep{pang2024iterative} are unable to overcome this shortcut, achieving test accuracy no better than \(1/d\). This failure is likely due to the difficulty transformer-based architectures face when unlearning spurious heuristics via policy-gradient optimization~\citep{hu2024learning}. In Table~\ref{tab:pita-star-graph}  we report test accuracies of PITA (ours) on three classes of graphs: smaller graphs \(\mathcal{G}(2, 5)\) and \(\mathcal{G}(5, 5)\), where we employ the GPT-2 small model, and a larger graph \(\mathcal{G}(3, 8)\), for which we use the GPT-2 medium model~\cite{radford2019language} to train the set of \textit{pre-trained models}.
%We report our test results .

\begin{table}[H]
    \centering
    \caption{Comparison of PITA with other baselines across star-graph configurations.}
    \label{tab:pita-star-graph}
    \begingroup
    \setlength{\tabcolsep}{6pt}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Algorithm} & $\mathcal{G}(2,5)$ & $\mathcal{G}(5,5)$ & $\mathcal{G}(3,8)$ \\
        \midrule
        pre-trained & 49.94 & 19.8 & 33.24 \\
        Q\# & 99.90 & 97 & 98.62 \\
        CD & 99.94 & 98.62 & 99.52 \\
        REINFORCE & 49.19 & 13.13 & 25.96 \\
        DPO & 37.61 & 0.0 & 0.0 \\
        RPO & 49.69 & 19.93 & 33.47 \\
        \midrule
        \textbf{PITA (ours)} & 99.97 & 99.7 & 99.93 \\
        \bottomrule
    \end{tabular}
    \endgroup
\end{table}




The star-graph experiments provide valuable insights into why PITA outperforms standard policy-based methods, as well as other value-based algorithms like Q\# and CD. While REINFORCE achieves a maximum accuracy of \(1/d\), the performance of DPO is significantly worse. We observe similar behavior to that reported in~\cite{zhou2025q}, where DPO achieves \(0\) accuracy, with the policy collapsing probabilities to \(0\). In contrast, value-based methods perform better across all graph configurations. Notably, PITA achieves further performance improvements, even when baseline reward-based methods are already near perfect accuracy. This improvement in accuracy can be attributed to PITA's ability to generate more precise implicit rewards. Upon examining the rewards generated by Q\# for the star-graph reasoning test set, we find that the reward differences between correct and incorrect answers are significantly smaller compared to those generated by PITA. Additional training details are provided in~\ref{app:experiments}

\subsection{Discussion}\label{subsec:discussion}

We empirically evaluate the proposed \textbf{PITA} algorithm for mathematical reasoning tasks, sentiment generation, and compare it against a strong reward-model baseline.

Our study focuses on three key questions: \textbf{(Q1)} Does PITA improve task accuracy (\textit{pass@1} and \textit{maj@8}) over a baseline using post-training Q\# with a learned preference reward model? \textbf{(Q2)} Does the KL divergence to the reference policy remain controlled? \textbf{(Q3)} How well does the learned reward model discriminate between correct and incorrect generations?

 We observe that PITA significantly outperforms the Q\#-HF baseline on both accuracy metrics while maintaining comparable or lower KL divergence. The poor performance of Q\#-HF can be attributed to the brittleness of its reward estimation process, which has failed to provide stable guidance during training. This demonstrates that iterative policy optimization with sparse rewards, as used in PITA, is more sample-efficient than single-stage MLE fine-tuning. PITA’s approach not only improves task performance but also reduces the need for large amounts of labeled preference data, making it more computationally efficient. Furthermore, PITA's ability to maintain alignment with the reference policy while improving accuracy highlights its robustness in real-world applications. Additional insights and tasks are presented in Appendix~\ref{app:experiments}.

%We observe that PITA outperforms the Q\#-HF baseline on both accuracy metrics while maintaining comparable or lower KL divergence, demonstrating that iterative policy optimization with sparse rewards is more sample-efficient than single-stage MLE fine-tuning. This suggests that PITA's approach to preference-guided learning is not only effective but also more computationally efficient, reducing the need for large amounts of labeled preference data. Furthermore, PITA's ability to maintain alignment with the reference policy while improving task performance highlights its robustness in real-world applications. Additional tasks are presented in Appendix~\ref{app:experiments}.

%We observe that PITA outperforms the Q\#-HF baseline on both accuracy metrics while maintaining comparable or lower KL divergence, demonstrating that iterative policy optimization with sparse rewards is more sample-efficient than single-stage MLE fine-tuning. Additional tasks are presented in Appendix~\ref{app:experiments}.
